PDETime: Rethinking Long-Term Multivariate Time Series Forecasting from the perspective of partial differential equations

Recent advancements in deep learning have led to the development of various models for long-term multivariate time-series forecasting (LMTF), many of which have shown promising results. Generally, the focus has been on historical-value-based models, which rely on past observations to predict future series. Notably, a new trend has emerged with time-index-based models, offering a more nuanced understanding of the continuous dynamics underlying time series. Unlike these two types of models that aggregate the information of spatial domains or temporal domains, in this paper, we consider multivariate time series as spatiotemporal data regularly sampled from a continuous dynamical system, which can be represented by partial differential equations (PDEs), with the spatial domain being fixed. Building on this perspective, we present PDETime, a novel LMTF model inspired by the principles of Neural PDE solvers, following the encoding-integration-decoding operations. Our extensive experimentation across seven diverse real-world LMTF datasets reveals that PDETime not only adapts effectively to the intrinsic spatiotemporal nature of the data but also sets new benchmarks, achieving state-of-the-art results

==> section/approach.tex <==
\section{Method}
\label{sec:approach}


\begin{figure}[!]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{icml2024/figure/framework.pdf}}\vspace{-3mm}
\caption{The framework of proposed PDETime which consists of an Encoder $E_{\theta}$, a Solver, and a Decoder $D_{\phi}$. Given the initial condition $x_{\tau_{0}}$, PDETime first simulates $\frac{\partial u(x,t_{\tau})}{\partial t_{\tau}}$ at each time step $t_{\tau}$ using the Encoder $E_{\theta}(x_{his},t_{\tau}, \tau)$; then uses the Solver to compute $\int_{\tau_{0}}^{\tau} \frac{\partial u(x,t_{\tau})}{\partial t_{\tau}} dt_{\tau} $, which is a numerical solver; finally, the Decoder maps integral term $z_{\tau}$ from latent space to special domains and predict the final results  $\hat{x}_{\tau}=x_{\tau_{0}}+D_{\phi}(z_{\tau})$. }
\label{fig:pdetime}
\end{center}\vspace{-3mm}
\vskip -0.2in
\end{figure}

%In this section, we outline the PDETime methodology, as depicted in Figure~\ref{fig:pdetime}, followed by a detailed examination of its individual components. The discussion culminates with an in-depth exploration of the objective function PDETime utilizes.

\subsection{Problem Formulation}
%\textbf{Problem setting} %Different from previous works~\cite{}, we treat multivariate time series as spatiotemporal 
%The multivariate dataset $u=[u_{1}(x,t),]$
In contrast to previous works~\cite{zhou2021informer, woo2023learning}, we regard multivariate time series as the spatiotemporal data regularly sampled from partial differential equations  along the temporal domain, which has the following form:
\begin{align}
    \mathcal{ F}(u, \frac{\partial u}{\partial t}, \frac{\partial u}{\partial x^{1}},..., \frac{\partial^{2} u}{\partial t^{2}},\frac{\partial^{2} u}{\partial x^{2}},...)=0, \nonumber \\
    u(x,t): \Omega \times \mathcal{T} \rightarrow \mathcal{V},
    \label{eq:pde_def}
\end{align}
subject to initial and boundary conditions. Here $u$ is a spatio-temporal dependent and multi-dimensional continuous vector field, $\Omega \in \mathbb{R}^{C}$ and $\mathcal{T} \in \mathbb{R}$ denote the spatial and temporal domains, respectively. For multivariate time series data, we regard channel attributes as spatial domains (e.g.,  the position and physical properties of sensors). 
The value of the spatial domains, $x$, is fixed but unknown (e.g., the position of sensors is fixed but unknown), while the value of the temporal domains is known.
%and the value of spatial domains $x$ is fixed and unknown. In contrast, the value of temporal domains is known. 
We treat LMTF as the Initial Value Problems, where $u(x_{t},t) \in \mathbb{R}^{C}$ at any time $t$ is required to infer $u(x_{t'},t') \in \mathbb{R}^{C}$.
%We present PDETime, a pioneering model for long-term multivariate time-series forecasting (LMTF) inspired by Partial Differential Equations (PDEs). Distinctively, PDETime conceptualizes LMTF challenges as Initial Value Problems (IVPs) within the framework of PDEs. Initially, we outline the PDETime methodology, as depicted in Figure~\ref{fig:pdetime}, followed by a detailed examination of its individual components. The discussion culminates with an in-depth exploration of the objective function PDETime utilizes.

%\subsection{Model Procedure}
%As mentioned in Section~\ref{sec:approach}, we treat the LMTF as Initial Value Problem. 

%PDETime conceptualizes LMTF challenges as Initial Value Problems within the framework of PDEs.
Consequently, we forecast the target series by the following formula: 
\begin{equation}
u(x,t)=u(x,t_{0})+\int_{t_{0}}^{t} \frac{\partial u(x,\tau)}{ \partial \tau} d\tau.
    \label{eq:pde}
\end{equation}

DETime initiates its process with a single initial condition, denoted as $u(x,t_{0})$, and leverages neural networks to project the system's dynamics forward in time. The procedure unfolds in three distinct steps. Firstly, PDETime generates a latent vector, $\alpha_{\tau}$ of a predefined dimension $d$, utilizing an encoder function, $E_{\theta}: \Omega \times \mathcal{T} \rightarrow \mathbb{R}^{d}$ (denoted as the ENC step). Subsequently, it employs an Euler solver, a numerical method, to approximate the integral term, $z_{t}=\int_{t_{0}}^{t} \alpha_{\tau} d\tau $, effectively capturing the system's evolution over time (denoted as the SOL step). In the final step, PDETime translates the latent vectors, 
$z_{t}$, back into the spatial domain using a decoder, 
 $D_{\phi}: \mathbb{R}^{d} \rightarrow \mathcal{V}$  to reconstruct the spatial function (denoted as the DEC step). This results in the following model, illustrated in Figure~\ref{fig:pdetime},
\begin{align}
    (ENC)\,\, \alpha_{\tau}&=E_{\theta}(x_{his}, t_{\tau},\tau)\\
    (SOL)\,\,\,\, z_{\tau}&=\int_{\tau_{0}}^{\tau} \alpha_{\tau} d\tau \\
    (DEC)\,\, x_{\tau}&=D_{\phi}(z_{\tau}) .
\end{align}
We describe the details of the components in Section~\ref{sec:component}.

\subsection{Components of PDETime}
\label{sec:component}

\subsubsection{Encoder: $\alpha_{\tau}=E_{\theta}(x_{his},t_{\tau},\tau)$}
\label{sec:forecaster}
The Encoder computes the latent vector $\alpha_{\tau}$ representing  $\frac{\partial u(x,t_{\tau})}{\partial t_{\tau}}$. 
In contrast to previous works~\cite{chen2022crom, yin2022continuous} that compute 
$\frac{\partial u(x,t_{\tau})}{\partial t_{\tau}}$ using auto-differentiation powered by deep learning frameworks, which often suffers from poor stability due to uncontrolled temporal discretizations,
%$\frac{\partial u(x,t_{\tau})}{\partial t_{\tau}}$ based on the auto-differentiation powered by deep learning frameworks, which suffers poor stability since the temporal discretizations are hardly controlled, 
we propose directly simulating $\frac{\partial u(x,t_{\tau})}{\partial t_{\tau}}$ by a carefully designed neural networks $E_{\theta} (x_{his},t_{\tau},\tau)$. 
The overall architecture of $E_{\theta} (x_{his},t_{\tau},\tau)$ is shown in Figure~\ref{fig:forecaster}. As mentioned in Section~\ref{sec:approach}, since the spatial domains of MTS data are fixed and unknown, we can only utilize the historical data $x_{his} \in \mathbb{R}^{H \times C}$ to assist the neural network in fitting the value of spatial domains $x$. 
To represent the high frequency of $\tau$, $x_{his}$, and $t_{\tau}$, we use concatenated Fourier Features (CFF)~\cite{woo2023learning, tancik2020fourier} and SIREN~\cite{sitzmann2020implicit} with $k$ layers.
%We use the concatenated Fourier Features (CFF)~\cite{woo2023learning, tancik2020fourier} and SIREN~\cite{sitzmann2020implicit} to represent high frequency of $\tau$, $x_{his}$, and $t_{\tau}$ with $k$ layers :
\begin{align}
    \tau^{(i)}&= \text{GELU}(W_{\tau}^{(i-1)}\tau^{(i-1)}+b_{\tau}^{(i-1)} )\nonumber \\
    x_{\tau}^{(i)}&= \sin(W_{x}^{(i-1)}x_{\tau}^{(i-1)}+b_{x}^{(i-1)}) \nonumber\\
    t_{\tau}^{(i)}&= \sin(W_{t}^{(i-1)}t_{\tau}^{(i-1)}+b_{t}^{(i-1)}), \,\,\, i=1,...,k 
\end{align}
where $x_{\tau}^{(0)} \in \mathbb{R}^{H \times C}=x_{his}$, $t_{\tau}^{(0)} \in \mathbb{R}^{t}$ is the temporal feature, and $\tau \in \mathbb{R}$ is the index feature where $\tau_{i}=\frac{i}{H+L}$ for $i=0,1,...,H+L$, $L$ and $H$ are the look-back and horizon length, respectively. We employ CFF to represent $\tau^{(0)}$, i.e. $\tau^{(0)}=[\sin(2\pi \textbf{B}_{1}\tau), \cos(2\pi \textbf{B}_{1}\tau),..., \sin(2 \pi \textbf{B}_{s} \tau), \cos (2 \pi \textbf{B}_{s} \tau)]$ where $\textbf{B}_{s} \in \mathbb{R}^{\frac{d}{2}\times c} $ is sampled from $\mathcal{N}(0,2^{s})$.
\par
After representing $\tau \in \mathbb{R}^{d}$, $t_{\tau} \in \mathbb{R}^{t}$, and $x_{\tau} \in \mathbb{R}^{d \times C}$ with INRs, the Encoder aggregates $x_{\tau}$ and $t_{\tau}$ using $\tau$, formulated as $f_{\theta}(\tau, t_{\tau},x_{\tau})$:
%uses $\tau$ to aggregate $x_{\tau}$ and $t_{\tau}$, which can be formulated as $f_{\theta}(\tau, t_{\tau},x_{\tau})$:
\begin{align}
    \tau&=\tau+\text{Attn}(\tau, x_{\tau}) \nonumber \\
    \tau&=\tau+\text{Linear}([\tau; t_{\tau}])
\end{align}
where $[\cdot;\cdot]$ is is the row-wise stacking operation. In this work, we utilize attention mechanism~\cite{vaswani2017attention} and linear mapping to aggregate the information of spatial domains and temporal domains, respectively. However, various networks can be designed to aggregate these two types of information.
\par
Unlike previous works~\cite{chen2022crom,yin2022continuous}, we do not directly make $\alpha_{\tau}=\frac{\partial u(x,t_{\tau})}{\partial t_{\tau}}$, but rather make $\int_{\tau_{0}}^{\tau}\alpha_{\tau} d \tau=\int_{\tau_{0}}^{\tau} \frac{\partial u(x, t_{\tau})}{\partial t_{\tau}} d \tau $ in latent space, without the need for autoregressive calculation of $\alpha_{t}$ which can effectively alleviate the error accumulation problem and make the prediction results more stable~\cite{brandstetter2021message}. 

The pseudocode of the Encoder of PDETime is summarized in Appendix~\ref{sec:code_Encoder}.


 

\begin{figure}[!]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=0.9\columnwidth]{icml2024/figure/Forecaster.pdf}}\vspace{-4mm}
\caption{The architecture of the Encoder which is used to simulate $\frac{\partial u(x,t_{\tau})}{\partial t_{\tau}}$. In this work, we use INRs to represent $x_{his}$, $t_{\tau}$, and $\tau$, and then use the Attention mechanism and linear mapping to aggregate the information of spatial domains and temporal domains.}
\label{fig:forecaster}
\end{center}\vspace{-2mm}
\vskip -0.2in
\end{figure}

\subsubsection{Solver: $z_{t}=\int_{\tau_{0}}^{\tau} \alpha_{\tau}$}
%\textbf{Estimator:} $z_{t}=\int_{\tau_{0}}^{\tau} \alpha_{\tau} d_{\tau}$. 
The Solver introduces a numerical solver (Euler Solver) to compute the integral term $z_{\tau}=\int_{\tau_{0}}^{\tau} \alpha_{\tau} d \tau$, which can be approximated as:
\begin{align}
    z_{\tau}&=\int_{\tau_{0}}^{\tau} \frac{\partial u(x_{\tau},t_{\tau})}{\partial t_{\tau}} d \tau \nonumber
    \approx \sum_{\tau=\tau_{0}}^{\tau}\frac{\partial u(x_{\tau}, t_{\tau})}{\partial t_{\tau}} \ast \Delta \tau \nonumber\\
    & \approx \sum_{\tau=\tau_{0}}^{\tau} E_{\theta}(x_{his},t_{\tau}, \tau) \ast \Delta \tau
    \label{eq:solver}
\end{align}
where we set $\Delta \tau=1$ for convenience. However, as shown in Figure~\ref{fig:est} (a), directly compute $z_{\tau}=\sum_{\tau=\tau_{0}}^{\tau} E_{\theta}(x_{his}, t_{\tau}, \tau) \ast \Delta \tau=\sum_{\tau=\tau_{0}}^{\tau} \alpha_{\tau} \ast \Delta \tau$ through Eq~\ref{eq:solver} can easily lead to error accumulation and gradient problems~\cite{rubanova2019latent,wu2022learning,brandstetter2021message}. To address these issues, we propose a modified approach, as illustrated in Figure~\ref{fig:est} (b). We divide the sequence into non-overlapping patches of length $S$, where $\frac{H+L}{S}$ patches are obtained. For $\tau(H+L) \mod S = 0$, we directly estimate the integral term as $z_{\tau} = f_{\psi}(x_{his},t_{\tau}, \tau)$ using a neural network $f_{\psi}$. Otherwise, we use the numerical solver to estimate the integral term with the integration lower limit $\lfloor \frac{\tau \cdot (H+L)}{S} \rfloor \cdot S$. This modification results in the following formula for the numerical solver:
% Therefore, in order to alleviate these problems, as shown in Figure~\ref{fig:est} (b), we first divide the sequence into $\frac{H+L}{S}$ non overlapping patches denoting the patch length as $S$. For $\tau(H+L) \mod S=0$, we directly estimate the integral term $z_{\tau}=f_{\psi}(x_{his},t_{\tau}, \tau)$ with a neural network $f_{\psi}$; otherwise, we use the numerical solver to estimate the integral term  with the integration lower bound $\lfloor \frac{\tau * (H+L)}{S} \rfloor \ast S$. Therefore, we modify the numerical solver to the following formula:
\begin{align}
    z_{t}&=f_{\psi}(x_{\tau'},t_{\tau'}, \tau')+\int_{\tau'}^{\tau}f_{\theta}(x_{\tau},t_{\tau}, \tau) d \tau,  \nonumber\\
    \tau'& =\lfloor \frac{\tau * (H+L)}{s} \rfloor \ast S
    \label{eq:new_numerical_solver}
\end{align}
% In addition, as shown in Figure~\ref{fig:est} (b), Eq~\ref{eq:new_numerical_solver} break the continuity of the integral term, therefore, we add the following objective function to ensure the continuity of the integral term as much as possible:
Furthermore, as shown in Figure~\ref{fig:est} (b), Eq~\ref{eq:new_numerical_solver} breaks the continuity. To address this, we introduce an additional objective function to ensure continuity as much as possible:
\begin{align}
    \mathcal{L}_{c}=\mathcal{L}(f_{\psi}(x_{\tau}, t_{\tau}, \tau),f_{\psi}(x_{\tau'}, t_{\tau'}, \tau')+\int_{\tau'}^{\tau}f_{\theta}(x_{\tau}, t_{\tau}, \tau) d \tau) \nonumber\\
    \mathrm{s.t.}\; \tau \ast(H+L) \mod S=0, \; \tau'=\frac{\tau\ast(L+H)-S}{(H+L)}.
\end{align}
The experimental results have shown that incorporating $\mathcal{L}_{c}$ improves the stability of PDETime. 

The pseudocode of the Solver of PDETime is summarized in Appendix~\ref{sec:code_Solver}.

\begin{figure}[!]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=0.9\columnwidth]{icml2024/figure/integral_3.pdf}}\vspace{-3mm}
\caption{The framework of standard and variant of numerical solver proposed in our work.}
\label{fig:est}
\end{center}\vspace{-2mm}
\vskip -0.2in
\end{figure}

\subsubsection{Decoder: $x_{\tau}=D_{\phi}(z_{\tau})+x_{\tau_{0}}$}
%\textbf{Decoder:} $x_{\tau}=D_{\phi}(z_{\tau})-x_{\tau_{0}}$. 
After estimating the integral term in latent space, we utilize a Decoder $D_{\phi}$ to decode $z_{\tau}$ into the spatial function. To tackle the distribution shift problem, we introduce a meta-optimization framework~\cite{woo2023learning,bertinetto2018meta} to enhance the extrapolation capability of PDETime. Specifically, we split the time series into look-back window $\textbf{X}_{t-L:t}=[x_{t-L},...,x_{t}] \in \mathbb{R}^{L \times C}$ and horizon window $\textbf{Y}_{t+1:t+H}=[x_{t+1},...,x_{t+H}] \in \mathbb{R}^{H \times C}$ pairs. We then use the parameters $\phi$ and $\theta$ to adapt the look-back window and horizon window through a bi-level problem:
%which is achieved by formulating the bi-level optimization problem:
\begin{align}
    \theta^{\ast}=\arg \min_{\theta} \sum_{\tau=\tau_{t+1}}^{\tau_{t+H}} \mathcal{L}_{p} ( D_{\phi}( \int_{\tau_{0}}^{\tau} E_{\theta}(x_{his},t_{\tau},\tau)),x_{\tau}) \nonumber \\
    \phi^{\ast}=\arg \min_{\phi} \sum_{\tau=\tau_{t-L}}^{\tau_{t}}\mathcal{L}_{r}( D_{\phi}( \int_{\tau_{0}}^{\tau} E_{\theta}(x_{his},t_{\tau},\tau)),x_{\tau})
\end{align}
where $\mathcal{L}_{r}$ and $\mathcal{L}_{p}$ denote the reconstruction and prediction loss, respectively (which will be described in detail in Section~\ref{sec:optimization}). During training, PDETime optimizes both $\theta$ and $\phi$; while during testing, it only optimizes $\phi$ to enhance the extrapolation. To ensure speed and efficiency, we employ a single ridge regression for $D_{\phi}$~\cite{bertinetto2018meta}.
%we set $D_{\phi}$ as a single ridge regression~\cite{bertinetto2018meta}.



% \begin{align}
%     \tau^{(0)}=[\sin(2\pi \textbf{B}_{1}\tau), \cos(2\pi \textbf{B}_{1}\tau),..., \sin(2 \pi \textbf{B}_{s} \tau), \cos (2 \pi \textbf{B}_{s} \tau)]
% \end{align}

% where $\textbf{B}_{s} \in \mathbb{R}^{\frac{d}{2}\times c} $ is sampled from $\mathcal{N}(0,2^{2s})$.


\subsection{Optimization}
\label{sec:optimization}
Different from previous works~\cite{zhou2021informer,zhou2022fedformer, wu2021autoformer,woo2023learning} that directly predict the future time steps with the objective $\mathcal{L}_{p}=\frac{1}{H}  \mathcal{L}(x_{\tau},\hat{x}_{\tau})$. As described as Eq~\ref{eq:pde}, we consider the LMTF as the Initial Value Problem in PDE, and the initial condition $x_{\tau_{0}}$is known (we use the latest time step in the historical series as the initial condition). Thus the objective of PDETime is to estimate the integral term $\int_{\tau_{0}}^{\tau}  \frac{\partial u(x,t_{\tau})}{\partial t_{\tau}} d\tau$. To achieve this, we define the prediction objective as:
\begin{align}
    \mathcal{L}_{p}=\frac{1}{H} \mathcal{L}(D_{\phi}(z_{\tau}),x_{\tau}-x_{\tau_{0}}) 
\end{align}
where $z_{\tau}=\int_{\tau_{0}}^{\tau} E_{\theta}(x_{his},t_{\tau},\tau) d\tau$ as described in Section~\ref{sec:forecaster}. Additionally, $\mathcal{L}_{r}$ has the same form $\mathcal{L}_{r}=\frac{1}{L} (D_{\phi}(z_{\tau}), x_{\tau}-x_{\tau_{0}})$.

% \begin{align}
%     z_{t}&=\int_{\tau_{0}}^{\tau_{1}} \frac{\partial u(x_{\tau},t_{\tau})}{\partial t_{\tau}} \nonumber\\
%     &\approx \sum_{\tau=\tau_{0}}^{\tau_{1}}\frac{\partial u(x_{\tau}, t_{\tau})}{\partial t_{\tau}} \ast \Delta \tau \nonumber\\
%     & \approx \sum_{\tau=\tau_{0}}^{\tau_{1}} f_{\theta}(x_{\tau},t_{\tau}, \tau) \ast \Delta \tau
% \end{align}
% \begin{align}
%     z_{t}&=f_{\psi}(x_{\tau'},t_{\tau'}, \tau')+\int_{\tau'}^{\tau}f_{\theta}(x_{\tau},t_{\tau}, \tau) d \tau,  \nonumber\\
%     \tau'& =\lfloor \frac{\tau * (H+P)}{s} \rfloor 
% \end{align}

% \begin{align}
%     f_{\psi}(x_{\tau}, t_{\tau}, \tau)=f_{\psi}(x_{\tau'}, t_{\tau'}, \tau')+\int_{\tau'}^{\tau}f_{\theta}(x_{\tau}, t_{\tau}, \tau) d \tau \nonumber\\
%     s.t.\,\, \tau \ast(L+P) \mod s=0, \,\, \tau'=\frac{\tau\ast(H+P)-s}{(H+P)}
% \end{align}
% \begin{align}
%     \mathcal{L}=\frac{1}{P}\sum_{\tau=\tau_{0}}^{\tau_{t_{0}+P}} \mathcal{L}(f_{\phi}(z_{\tau}),x_{\tau}-x_{\tau_{0}}) 
% \end{align}

In addition to the prediction objective, we also aim to ensure that the first-order difference of the predicted sequence matches that of the target sequence. Therefore, we introduce the optimization objective:
%Furthermore, we aim for the first-order difference of the predicted sequence to be equal to that of the target sequence. Therefore, we  also have the following optimization objective:
\begin{align}
    \mathcal{L}_{f}=\frac{1}{H} \sum_{\tau=\tau_{t+1}}^{\tau_{t+H}} \mathcal{L}(D_{\phi}(z_{\tau})-D_{\phi}(z_{\tau-1}),x_{\tau}-x_{\tau-1})
\end{align}
Combining $\mathcal{L}_{p}$, $\mathcal{L}_{c}$, and $\mathcal{L}_{f}$, the training objective is:
\begin{align}
\mathcal{L}_{p}=\mathcal{L}_{p}+\mathcal{L}_{c}+\mathcal{L}_{f}.
\end{align}
%where $\mathcal{L}_{p}=\frac{1}{H} %\sum_{\tau=\tau_{0}}^{\tau_{H}}\mathcal{L}(x_{\tau}, \hat{x}_{\tau})$
% \begin{algorithm}
% \caption{PDETime training}
% \begin{algorithmic}
%     \REQUIRE Training set $S$ \\
%     \REQUIRE Learning rate $\alpha$, $\beta$ \\
%     \REQUIRE Randomly initialize $\theta$, $\psi$, $\phi$ \\
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[ht!]  %ht!参数是调整算法在文章中的位置
% 	%	\renewcommand{\algorithmicrequire}{\textbf{Input  \ \ :}}  %这样的指令可以让output和input的‘:’号在同一竖线上。但没必要，所以我注释了
% 	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
% 	\renewcommand{\algorithmicensure}{\textbf{Output:}}
% 	\caption{PDETime Training}  
% 	\label{alg:}
% 	\begin{algorithmic}[1] %每行显示行号
% 		% \Require Faulty program  ($\textit{P}$)
% 		% \Require Test cases $\left(\textit{Tests}\right) $
% 		% \Require xxx 
% 		% \Require xxx %细节就不多说了，略之
% 		% \Ensure  xxx 
%         \Require Training set $S$
%         \Require Learning rate $\alpha$, $\beta$
%         \Require Randomly initialize $\theta$, $\psi$, $\phi$
%         %\State \textbf{While} no convergence \textbf{do}
%         \While{no convergence}
%         \State Sample batch $\mathcal{B}$ from $\mathcal{S}$ of data $(s^{(j)})_{j \in \mathcal{B}}$ 
        
		
% 		\Function{xxx}{xxx} \label{xxx1}
% 		\For{xxx} 
% 		\myState{xxx} 
% 		\State xxx
% 		\EndFor 
% 		\EndFunction \label{xxx2}
		
% 		\Statex   %算法中的空行
		
% 		\Function{main}{}
% 		\State xxx
% 		\Repeat
% 			\If{xxx}
% 				\State xxx
% 			\Else  \Comment{xxx}  %注释
% 				\State xxx
% 				\For{xxx} 
% 					\If{xxx}
% 						\State xxx
% 					\EndIf
% 				\EndFor
% 				\State xxx
% 			\EndIf
			
% 		   	\State xxx
% 			\If{xxx}
% 				\State xxx
% 			\EndIf
% 		\Until{xxx}
% 		\EndFunction
% 	\end{algorithmic}
% \end{algorithm}


%\begin{equation}
%    z_{t}=f_{\psi}(x_{\tau'},t_{\tau'}, \tau')+\int_{\tau'}^{\tau}f_{\theta}(x_{\tau}, \\t_{\tau}, \tau) d \tau , \tau'=\lfloor \frac{\tau * (H+P)}{s} \rfloor 
%\end{equation}

==> section/conclusion.tex <==
\section{Conclusion and Future Work}
In this paper, we propose a novel LMTS framework PDETime, based on neural PDE solvers, which consists of Encoder, Solver, and Decoder. Specifically, the Encoder simulates the partial differentiation of the original function over time at each time step in latent space in parallel. 
%The Solver is a numerical solver that compute the integral term with a more stable performance. 
The solver is responsible for computing the integral term with improved stability. 
Finally, the Decoder maps the integral term from latent space into the spatial function and predicts the target series given the initial condition. 
%Like time-index-based models, we also utilize the meta-optimization to enhance the ability to extrapolate future series.
Additionally, we incorporate meta-optimization techniques to enhance the ability of PDETime to extrapolate future series.
Extensive experimental results show that PDETime achieves state-of-the-art performance across forecasting benchmarks on various real-world datasets. We also perform ablation studies to identify the key components contributing to the success of PDETime. 

% \textbf{Future Work} Inspired by partial differential equations, we first propose a neural PDE solver, named PDETime, to long-term multivariate time-series forecasting and have achieved competitive or even better performance. In fact, neural PDE solvers have been fully developed and have made great progress in PDE related tasks. Whether other types of neural PDE solvers can be applied to LMTF is an interesting future direction. In addition, ablation studies have found that the effectiveness of special domains (historical observations) on PDETime is limited, and the impact of temporal domains on PDETime various significantly across different datasets, therefore, how to design effective network structures to better utilizing spatial and temporal domains is also an important future work. 
% Moreover, neural PDE solvers have a strong ability to handle irregular series, thus another potential future direction is applying PDETime to irregular time series related tasks like missing value imputation. Finally, different from historical-value-based and time-index-based models, we rethink LMTS forecasting task from the perspective of PDEs, and have achieved SOTA performance, and rethinking the LTMS forecasting from various perspective is a promising direction.

\textbf{Future Work} Firstly, while our proposed neural PDE solver, PDETime, has shown promising results for long-term multivariate time series forecasting, there are other types of neural PDE solvers that could potentially be applied to this task. Exploring these alternative neural PDE solvers and comparing their performance on LMTF could be an interesting future direction. 
Furthermore, our ablation studies have revealed that the effectiveness of the historical observations (spatial domain) on PDETime is limited, and the impact of the temporal domain varies significantly across different datasets. Designing effective network structures that better utilize the spatial and temporal domains could be an important area for future research. 
%Additionally, neural PDE solvers have demonstrated strong capabilities in handling irregular time series data. Therefore, another potential future direction is to apply PDETime to irregular time series tasks, such as missing value imputation. 
Finally, our approach of rethinking long-term multivariate time series forecasting from the perspective of partial differential equations has led to state-of-the-art performance. Exploring other perspectives and frameworks to tackle this task could be a promising direction for future research.





==> section/experiment.tex <==
\section{Experiments}
\subsection{Experimental Settings}
\textbf{Datasets.} We extensively include 7 real-world datasets in our experiments, including four ETT datasets (ETTh1, ETTh2, ETTm1, ETTm2)~\cite{zhou2021informer}. Electricity, Weather and Traffic~\cite{wu2021autoformer}, covering energy, transportation and weather domains (See Appendix~\ref{sec:dataset_details} for more details on the datasets). To ensure a fair evaluation, we follow the standard protocol of dividing each dataset into the training, validation and testing subsets according to the chronological order. The split ratio is 6:2:2 for the ETT dataset and 7:1:2 for the others~\cite{zhou2021informer,wu2021autoformer}. We set the length of the lookback series as 512 for PatchTST, 336 for DLinear, and 96 for other historical-value-based models. The experimental settings of DeepTime remain consistent with the original settings~\cite{woo2023learning}. 
%The experimental settings of DeepTime follows the original settings of DeepTime~\cite{woo2023learning}. 
The prediction length varies in $\{ 96, 192, 336, 720 \}$. 

\textbf{Comparison methods.} We carefully choose 10 well-acknowledged models (9 historical-value-based models and 1 time-index-based model) as our benchmarks, including (1) Transformer-based models: Autoformer~\cite{wu2021autoformer}, FEDformer~\cite{zhou2022fedformer}, Stationary~\cite{liu2022non}, Crossformer~\cite{zhang2022crossformer}, PatchTST~\cite{nie2022time}, and iTransformer~\cite{liu2023itransformer}; (2) Linear-based models: DLinear~\cite{zeng2023transformers} ; (3) CNN-based models: SCINet~\cite{liu2022scinet}, TimesNet~\cite{wu2022timesnet}; (4) Time-index-based model: DeepTime~\cite{woo2023learning}. (See Appendix~\ref{baselines_details} for details of these baselines)


\textbf{Implementation Details.} Our method is trained with the Smooth L1~\cite{girshick2015fast} loss using the ADAM~\cite{kingma2014adam} with the initial learning rate selected from $\{10^{-4},10^{-3}, 5\times 10^{-3} \}$. Batch size is set to 32. All experiments are repeated 3 times with fixed seed 2024, implemented in Pytorch~\cite{paszke2019pytorch} and conducted on a single NVIDIA RTX 3090 GPUs. Following DeepTime~\cite{woo2023learning}, we set the look-back length as $L=\mu \ast H$, where $\mu$ is a multiplier which decides the length of the look-back windows. We search through the values $\mu =[1,3,5,7,9]$, and select the best value based on the validation loss.
We set layers of INRs $k=5$ by default, and select the best results from $N=\{ 1,2,3,5\}$. We summarize the temporal features used in this work in Appendix~\ref{sec:time_features}.

\subsection{Main Results and Ablation Study}

\begin{table*}[!]
  \caption{\update{Full results of the long-term forecasting task}. We compare extensive competitive models under different prediction lengths following the setting of PatchTST~\citeyearpar{nie2022time}. The input sequence length is set to 336 and 512 for DLinear and PatchTST, and 96 for other historical-value-based baselines. \emph{Avg} means the average results from all four prediction lengths.}\label{tab:full_baseline_results}
  \vskip -0.0in
  \vspace{3pt}
  \renewcommand{\arraystretch}{0.85} 
  \centering
  %\resizebox{1\columnwidth}{!}{
  \begin{threeparttable}
  \begin{small}
  \renewcommand{\multirowsetup}{\centering}
  \setlength{\tabcolsep}{2.5pt}
  \begin{tabular}{c|c|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc}
    \toprule
    \multicolumn{2}{c}{\multirow{2}{*}{Models}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{\textbf{PDETime}}}} &
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{{iTransformer}}}} &
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{{PatchTST}}}} &
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Crossformer}}}  &
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{{DeepTime}}}} &
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{{TimesNet}}}} &
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{{DLinear}}}}&
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{SCINet}}} &
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{FEDformer}}} &
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Stationary}}} &
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Autoformer}}} \\
    %&\multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Informer}}} 
    \multicolumn{2}{c}{} &
    \multicolumn{2}{c}{\scalebox{0.8}{\textbf{(Ours)}}} & 
    \multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{liu2023itransformer}}} & 
    \multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{nie2022time}}} & 
    \multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{zhang2022crossformer}}}  & 
    \multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{woo2023learning}}} & 
    \multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{wu2022timesnet}}} & 
    \multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{zeng2023transformers}}}& 
    \multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{liu2022scinet}}} &
    \multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{zhou2022fedformer}}} &
    \multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{liu2022non}}} &
    \multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{wu2021autoformer}}} \\
    %&\multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{Informer}}} 
    \cmidrule(lr){3-4} \cmidrule(lr){5-6}\cmidrule(lr){7-8} \cmidrule(lr){9-10}\cmidrule(lr){11-12}\cmidrule(lr){13-14} \cmidrule(lr){15-16} \cmidrule(lr){17-18} \cmidrule(lr){19-20} \cmidrule(lr){21-22} \cmidrule(lr){23-24}
    \multicolumn{2}{c}{Metric}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} \\
    \toprule
    
    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{ETTm1}}}
    &  \scalebox{0.78}{96} & \textbf{\scalebox{0.78}{0.292}} & \textbf{\scalebox{0.78}{0.335}} & \scalebox{0.78}{0.334} & \scalebox{0.78}{0.368} & \underline{\scalebox{0.78}{0.293}} & {\scalebox{0.78}{0.346}} & \scalebox{0.78}{0.404} & \scalebox{0.78}{0.426} & \scalebox{0.78}{0.305} & \scalebox{0.78}{0.347} &{\scalebox{0.78}{0.338}} &{\scalebox{0.78}{0.375}} &{\scalebox{0.78}{0.299}} &\underline{\scalebox{0.78}{0.343}} & \scalebox{0.78}{0.418} & \scalebox{0.78}{0.438} &\scalebox{0.78}{0.379} &\scalebox{0.78}{0.419} &\scalebox{0.78}{0.386} &\scalebox{0.78}{0.398} &\scalebox{0.78}{0.505} &\scalebox{0.78}{0.475} \\ %&\scalebox{0.78}{0.672} &\scalebox{0.78}{0.571} \\
    & \scalebox{0.78}{192} & \textbf{\scalebox{0.78}{0.329}} & \textbf{\scalebox{0.78}{0.359}} & \scalebox{0.78}{0.377} & \scalebox{0.78}{0.391} & \underline{\scalebox{0.78}{0.333}} & {\scalebox{0.78}{0.370}} & \scalebox{0.78}{0.450} & \scalebox{0.78}{0.451} &\scalebox{0.78}{0.340} & \scalebox{0.78}{0.371} &{\scalebox{0.78}{0.374}} &{\scalebox{0.78}{0.387}}  &{\scalebox{0.78}{0.335}} &\underline{\scalebox{0.78}{0.365}} & \scalebox{0.78}{0.439} & \scalebox{0.78}{0.450}  &\scalebox{0.78}{0.426} &\scalebox{0.78}{0.441} &\scalebox{0.78}{0.459} &\scalebox{0.78}{0.444} &\scalebox{0.78}{0.553} &\scalebox{0.78}{0.496} \\ %&\scalebox{0.78}{0.795} &\scalebox{0.78}{0.669}\\
    & \scalebox{0.78}{336} & \textbf{\scalebox{0.78}{0.346}} & \textbf{\scalebox{0.78}{0.374}} & \scalebox{0.78}{0.426} & \scalebox{0.78}{0.420} & {\scalebox{0.78}{0.369}} & {\scalebox{0.78}{0.392}} & \scalebox{0.78}{0.532}  &\scalebox{0.78}{0.515} & \underline{\scalebox{0.78}{0.362}} & \scalebox{0.78}{0.387} &{\scalebox{0.78}{0.410}} &{\scalebox{0.78}{0.411}}  &{\scalebox{0.78}{0.369}} &\underline{\scalebox{0.78}{0.386}} & \scalebox{0.78}{0.490} & \scalebox{0.78}{0.485}  &\scalebox{0.78}{0.445} &\scalebox{0.78}{0.459} &\scalebox{0.78}{0.495} &\scalebox{0.78}{0.464} &\scalebox{0.78}{0.621} &\scalebox{0.78}{0.537} \\ %&\scalebox{0.78}{1.212} &\scalebox{0.78}{0.871} \\
    & \scalebox{0.78}{720} & \textbf{\scalebox{0.78}{0.395}} & \textbf{\scalebox{0.78}{0.404}} & \scalebox{0.78}{0.491} & \scalebox{0.78}{0.459} & {\scalebox{0.78}{0.416}} & {\scalebox{0.78}{0.420}} & \scalebox{0.78}{0.666} & \scalebox{0.78}{0.589} & \underline{\scalebox{0.78}{0.399}} & \underline{\scalebox{0.78}{0.414}} &{\scalebox{0.78}{0.478}} &{\scalebox{0.78}{0.450}} &{\scalebox{0.78}{0.425}} &{\scalebox{0.78}{0.421}} & \scalebox{0.78}{0.595} & \scalebox{0.78}{0.550}  &\scalebox{0.78}{0.543} &\scalebox{0.78}{0.490} &\scalebox{0.78}{0.585} &\scalebox{0.78}{0.516} &\scalebox{0.78}{0.671} &\scalebox{0.78}{0.561} \\ %&\scalebox{0.78}{1.166} &\scalebox{0.78}{0.823} \\
    \cmidrule(lr){2-24}
    & \scalebox{0.78}{Avg} & \textbf{\scalebox{0.78}{0.340}} & \textbf{\scalebox{0.78}{0.368}} & \scalebox{0.78}{0.407} & \scalebox{0.78}{0.410} & {\scalebox{0.78}{0.352}} & {\scalebox{0.78}{0.382}} & \scalebox{0.78}{0.513} & \scalebox{0.78}{0.496} & \underline{\scalebox{0.78}{0.351}} & \scalebox{0.78}{0.379} &{\scalebox{0.78}{0.400}} &{\scalebox{0.78}{0.406}}  &{\scalebox{0.78}{0.357}} &\underline{\scalebox{0.78}{0.378}} & \scalebox{0.78}{0.485} & \scalebox{0.78}{0.481}  &\scalebox{0.78}{0.448} &\scalebox{0.78}{0.452} &\scalebox{0.78}{0.481} &\scalebox{0.78}{0.456} &\scalebox{0.78}{0.588} &\scalebox{0.78}{0.517} \\ %&\scalebox{0.78}{0.961} &\scalebox{0.78}{0.734} \\
    \midrule
    
    \multirow{5}{*}{\update{\rotatebox{90}{\scalebox{0.95}{ETTm2}}}}
    &  \scalebox{0.78}{96} & \textbf{\scalebox{0.78}{0.158}} & \textbf{\scalebox{0.78}{0.244}} & \scalebox{0.78}{0.180} & \scalebox{0.78}{0.264} & \underline{\scalebox{0.78}{0.166}} & \underline{{\scalebox{0.78}{0.256}}} & \scalebox{0.78}{0.287} & \scalebox{0.78}{0.366} & \underline{\scalebox{0.78}{0.166}} & \scalebox{0.78}{0.257} &{\scalebox{0.78}{0.187}} &\scalebox{0.78}{0.267} &\scalebox{0.78}{0.167} &\scalebox{0.78}{0.260} & \scalebox{0.78}{0.286} & \scalebox{0.78}{0.377} &\scalebox{0.78}{0.203} &\scalebox{0.78}{0.287} &{\scalebox{0.78}{0.192}} &\scalebox{0.78}{0.274} &\scalebox{0.78}{0.255} &\scalebox{0.78}{0.339} \\ % &\scalebox{0.78}{0.365} &\scalebox{0.78}{0.453} \\
    & \scalebox{0.78}{192} & \textbf{\scalebox{0.78}{0.213}} & \textbf{\scalebox{0.78}{0.283}} & {\scalebox{0.78}{0.250}} & {\scalebox{0.78}{0.309}} & \underline{\scalebox{0.78}{0.223}} & \underline{\scalebox{0.78}{0.296}} & \scalebox{0.78}{0.414} & \scalebox{0.78}{0.492} & \scalebox{0.78}{0.225} & \scalebox{0.78}{0.302} &{\scalebox{0.78}{0.249}} &{\scalebox{0.78}{0.309}} &\scalebox{0.78}{0.224} &\scalebox{0.78}{0.303} & \scalebox{0.78}{0.399} & \scalebox{0.78}{0.445} &\scalebox{0.78}{0.269} &\scalebox{0.78}{0.328} &\scalebox{0.78}{0.280} &\scalebox{0.78}{0.339} &\scalebox{0.78}{0.281} &\scalebox{0.78}{0.340} \\ %&\scalebox{0.78}{0.533} &\scalebox{0.78}{0.563} \\
    & \scalebox{0.78}{336} & \textbf{\scalebox{0.78}{0.262}} & \textbf{\scalebox{0.78}{0.318}} & {\scalebox{0.78}{0.311}} & {\scalebox{0.78}{0.348}} & \underline{\scalebox{0.78}{0.274}} & \underline{\scalebox{0.78}{0.329}}  & \scalebox{0.78}{0.597} & \scalebox{0.78}{0.542}  & \scalebox{0.78}{0.277} & \scalebox{0.78}{0.336} &{\scalebox{0.78}{0.321}} &{\scalebox{0.78}{0.351}} &\scalebox{0.78}{0.281} &\scalebox{0.78}{0.342} & \scalebox{0.78}{0.637} & \scalebox{0.78}{0.591} &\scalebox{0.78}{0.325} &\scalebox{0.78}{0.366} &\scalebox{0.78}{0.334} &\scalebox{0.78}{0.361} &\scalebox{0.78}{0.339} &\scalebox{0.78}{0.372} \\ %&\scalebox{0.78}{1.363} &\scalebox{0.78}{0.887} \\
    & \scalebox{0.78}{720} & \textbf{\scalebox{0.78}{0.334}} & \textbf{\scalebox{0.78}{0.336}} & {\scalebox{0.78}{0.412}} & {\scalebox{0.78}{0.407}} & \underline{\scalebox{0.78}{0.362}} & \underline{\scalebox{0.78}{0.385}} & \scalebox{0.78}{1.730} & \scalebox{0.78}{1.042} & \scalebox{0.78}{0.383} & \scalebox{0.78}{0.409} &{\scalebox{0.78}{0.408}} &{\scalebox{0.78}{0.403}} &\scalebox{0.78}{0.397} &\scalebox{0.78}{0.421} & \scalebox{0.78}{0.960} & \scalebox{0.78}{0.735} &\scalebox{0.78}{0.421} &\scalebox{0.78}{0.415} &\scalebox{0.78}{0.417} &\scalebox{0.78}{0.413} &\scalebox{0.78}{0.433} &\scalebox{0.78}{0.432} \\ %&\scalebox{0.78}{3.379} &\scalebox{0.78}{1.338} \\
    \cmidrule(lr){2-24}
    & \scalebox{0.78}{Avg} & \textbf{\scalebox{0.78}{0.241}} & \textbf{\scalebox{0.78}{0.295}} & {\scalebox{0.78}{0.288}} & {\scalebox{0.78}{0.332}} & \underline{\scalebox{0.78}{0.256}} & \underline{\scalebox{0.78}{0.316}} & \scalebox{0.78}{0.757} & \scalebox{0.78}{0.610} & \scalebox{0.78}{0.262} & \scalebox{0.78}{0.326} &{\scalebox{0.78}{0.291}} &{\scalebox{0.78}{0.333}} &\scalebox{0.78}{0.267} &\scalebox{0.78}{0.331} & \scalebox{0.78}{0.571} & \scalebox{0.78}{0.537} &\scalebox{0.78}{0.305} &\scalebox{0.78}{0.349} &\scalebox{0.78}{0.306} &\scalebox{0.78}{0.347} &\scalebox{0.78}{0.327} &\scalebox{0.78}{0.371} \\ %&\scalebox{0.78}{1.410} &\scalebox{0.78}{0.810} \\
    \midrule
    
    \multirow{5}{*}{\rotatebox{90}{\update{\scalebox{0.95}{ETTh1}}}}
    &  \scalebox{0.78}{96} & \textbf{\scalebox{0.78}{0.356}} & \textbf{\scalebox{0.78}{0.381}} & \scalebox{0.78}{0.386} & {\scalebox{0.78}{0.405}} & \scalebox{0.78}{0.379} & \scalebox{0.78}{0.401} & \scalebox{0.78}{0.423} & \scalebox{0.78}{0.448} & \underline{\scalebox{0.78}{0.371}}& \underline{\scalebox{0.78}{0.396}}  &{\scalebox{0.78}{0.384}} &{\scalebox{0.78}{0.402}} & \scalebox{0.78}{0.375} &{\scalebox{0.78}{0.399}} & \scalebox{0.78}{0.654} & \scalebox{0.78}{0.599} &{\scalebox{0.78}{0.376}} &\scalebox{0.78}{0.419} &\scalebox{0.78}{0.513} &\scalebox{0.78}{0.491} &\scalebox{0.78}{0.449} &\scalebox{0.78}{0.459}  \\ %&\scalebox{0.78}{0.865} &\scalebox{0.78}{0.713} \\
    & \scalebox{0.78}{192} & \textbf{\scalebox{0.78}{0.397}} & \textbf{\scalebox{0.78}{0.406}} & {\scalebox{0.78}{0.441}} & {\scalebox{0.78}{0.436}} & \scalebox{0.78}{0.413} & \scalebox{0.78}{0.429} & \scalebox{0.78}{0.471} & \scalebox{0.78}{0.474}  & \underline{\scalebox{0.78}{0.403}} & \underline{\scalebox{0.78}{0.420}} &{\scalebox{0.78}{0.436}} &{\scalebox{0.78}{0.429}}  &{\scalebox{0.78}{0.405}} &{\scalebox{0.78}{0.416}} & \scalebox{0.78}{0.719} & \scalebox{0.78}{0.631} &{\scalebox{0.78}{0.420}} &\scalebox{0.78}{0.448} &\scalebox{0.78}{0.534} &\scalebox{0.78}{0.504} &\scalebox{0.78}{0.500} &\scalebox{0.78}{0.482} \\ %&\scalebox{0.78}{1.008} &\scalebox{0.78}{0.792} \\
    & \scalebox{0.78}{336} & \textbf{\scalebox{0.78}{0.420}} & \textbf{\scalebox{0.78}{0.419}} & {\scalebox{0.78}{0.487}} & {\scalebox{0.78}{0.458}} & \scalebox{0.78}{0.435} & \underline{\scalebox{0.78}{0.436}} & \scalebox{0.78}{0.570} & \scalebox{0.78}{0.546} & \underline{\scalebox{0.78}{0.433}} & \underline{\scalebox{0.78}{0.436}} &\scalebox{0.78}{0.491} &\scalebox{0.78}{0.469} &{\scalebox{0.78}{0.439}} & {\scalebox{0.78}{0.443}} & \scalebox{0.78}{0.778} & \scalebox{0.78}{0.659} & {\scalebox{0.78}{0.459}} &{\scalebox{0.78}{0.465}} &\scalebox{0.78}{0.588} &\scalebox{0.78}{0.535} &\scalebox{0.78}{0.521} &\scalebox{0.78}{0.496} \\ %&\scalebox{0.78}{1.107} &\scalebox{0.78}{0.809} \\
    & \scalebox{0.78}{720} & \textbf{\scalebox{0.78}{0.425}} & \textbf{\scalebox{0.78}{0.446}} & {\scalebox{0.78}{0.503}} & 
    {\scalebox{0.78}{0.491}} & \underline{\scalebox{0.78}{0.446}} & \underline{\scalebox{0.78}{0.464}} & \scalebox{0.78}{0.653} & \scalebox{0.78}{0.621} & \scalebox{0.78}{0.474} & \scalebox{0.78}{0.492} &\scalebox{0.78}{0.521} &{\scalebox{0.78}{0.500}} &\scalebox{0.78}{0.472} &\scalebox{0.78}{0.490} & \scalebox{0.78}{0.836} & \scalebox{0.78}{0.699} &{\scalebox{0.78}{0.506}} &{\scalebox{0.78}{0.507}} &\scalebox{0.78}{0.643} &\scalebox{0.78}{0.616} &{\scalebox{0.78}{0.514}} &\scalebox{0.78}{0.512}  \\ %&\scalebox{0.78}{1.181} &\scalebox{0.78}{0.865} \\
    \cmidrule(lr){2-24}
    & \scalebox{0.78}{Avg} & \textbf{\scalebox{0.78}{0.399}} & \textbf{\scalebox{0.78}{0.413}} & {\scalebox{0.78}{0.454}} & {\scalebox{0.78}{0.447}} & \underline{\scalebox{0.78}{0.418}} & \underline{\scalebox{0.78}{0.432}} & \scalebox{0.78}{0.529} & \scalebox{0.78}{0.522} & \scalebox{0.78}{0.420} & \scalebox{0.78}{0.436} &\scalebox{0.78}{0.458} &{\scalebox{0.78}{0.450}} &{\scalebox{0.78}{0.423}} &{\scalebox{0.78}{0.437}} & \scalebox{0.78}{0.747} & \scalebox{0.78}{0.647} &{\scalebox{0.78}{0.440}} &\scalebox{0.78}{0.460} &\scalebox{0.78}{0.570} &\scalebox{0.78}{0.537} &\scalebox{0.78}{0.496} &\scalebox{0.78}{0.487}  \\ %&\scalebox{0.78}{1.040} &\scalebox{0.78}{0.795} \\
    \midrule

    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{ETTh2}}}
    &  \scalebox{0.78}{96} & \textbf{\scalebox{0.78}{0.268}} & \textbf{\scalebox{0.78}{0.330}} & {\scalebox{0.78}{0.297}} & {\scalebox{0.78}{0.349}} & \underline{\scalebox{0.78}{0.274}} & \underline{\scalebox{0.78}{0.335}} & \scalebox{0.78}{0.745} & \scalebox{0.78}{0.584} &\scalebox{0.78}{0.287} & \scalebox{0.78}{0.352}  & {\scalebox{0.78}{0.340}} & {\scalebox{0.78}{0.374}} &{\scalebox{0.78}{0.289}} &{\scalebox{0.78}{0.353}} & \scalebox{0.78}{0.707} & \scalebox{0.78}{0.621}  &\scalebox{0.78}{0.358} &\scalebox{0.78}{0.397} &\scalebox{0.78}{0.476} &\scalebox{0.78}{0.458} &\scalebox{0.78}{0.346} &\scalebox{0.78}{0.388} \\ %&\scalebox{0.78}{3.755} &\scalebox{0.78}{1.525} \\
    & \scalebox{0.78}{192} & \textbf{\scalebox{0.78}{0.331}} & \textbf{\scalebox{0.78}{0.370}} & {\scalebox{0.78}{0.380}} & {\scalebox{0.78}{0.400}} &\underline{\scalebox{0.78}{0.342}} & \underline{\scalebox{0.78}{0.382}} & \scalebox{0.78}{0.877} & \scalebox{0.78}{0.656} & \scalebox{0.78}{0.383} & \scalebox{0.78}{0.412} & {\scalebox{0.78}{0.402}} & {\scalebox{0.78}{0.414}} &\scalebox{0.78}{0.383} &\scalebox{0.78}{0.418} & \scalebox{0.78}{0.860} & \scalebox{0.78}{0.689} &{\scalebox{0.78}{0.429}} &{\scalebox{0.78}{0.439}} &\scalebox{0.78}{0.512} &\scalebox{0.78}{0.493} &\scalebox{0.78}{0.456} &\scalebox{0.78}{0.452} \\ %&\scalebox{0.78}{5.602} &\scalebox{0.78}{1.931} \\
    & \scalebox{0.78}{336} & \textbf{\scalebox{0.78}{0.358}} & \textbf{\scalebox{0.78}{0.395}} & {\scalebox{0.78}{0.428}} & {\scalebox{0.78}{0.432}} & \underline{\scalebox{0.78}{0.365}} & \underline{\scalebox{0.78}{0.404}}& \scalebox{0.78}{1.043} & \scalebox{0.78}{0.731} & \scalebox{0.78}{0.523} & \scalebox{0.78}{0.501}  & {\scalebox{0.78}{0.452}} & {\scalebox{0.78}{0.452}} &\scalebox{0.78}{0.448} &\scalebox{0.78}{0.465} & \scalebox{0.78}{1.000} &\scalebox{0.78}{0.744} &\scalebox{0.78}{0.496} &\scalebox{0.78}{0.487} &\scalebox{0.78}{0.552} &\scalebox{0.78}{0.551} &{\scalebox{0.78}{0.482}} &\scalebox{0.78}{0.486}\\ % &\scalebox{0.78}{4.721} &\scalebox{0.78}{1.835} \\
    & \scalebox{0.78}{720} & \textbf{\scalebox{0.78}{0.380}} & \textbf{\scalebox{0.78}{0.421}} & {\scalebox{0.78}{0.427}} & {\scalebox{0.78}{0.445}} & \underline{\scalebox{0.78}{0.393}} & \underline{\scalebox{0.78}{0.430}} & \scalebox{0.78}{1.104} & \scalebox{0.78}{0.763} & \scalebox{0.78}{0.765} & \scalebox{0.78}{0.624} & {\scalebox{0.78}{0.462}} & {\scalebox{0.78}{0.468}} &\scalebox{0.78}{0.605} &\scalebox{0.78}{0.551} & \scalebox{0.78}{1.249} & \scalebox{0.78}{0.838} &{\scalebox{0.78}{0.463}} &{\scalebox{0.78}{0.474}} &\scalebox{0.78}{0.562} &\scalebox{0.78}{0.560} &\scalebox{0.78}{0.515} &\scalebox{0.78}{0.511} \\ %&\scalebox{0.78}{3.647} &\scalebox{0.78}{1.625} \\
    \cmidrule(lr){2-24}
    & \scalebox{0.78}{Avg} & \textbf{\scalebox{0.78}{0.334}} & \textbf{\scalebox{0.78}{0.379}} & {\scalebox{0.78}{0.383}} & {\scalebox{0.78}{0.407}} & \underline{\scalebox{0.78}{0.343}} & \underline{\scalebox{0.78}{0.387}} & \scalebox{0.78}{0.942} & \scalebox{0.78}{0.684} & \scalebox{0.78}{0.489} & \scalebox{0.78}{0.472}  &{\scalebox{0.78}{0.414}} &{\scalebox{0.78}{0.427}} &\scalebox{0.78}{0.431} &\scalebox{0.78}{0.446} & \scalebox{0.78}{0.954} & \scalebox{0.78}{0.723} &\scalebox{0.78}{{0.437}} &\scalebox{0.78}{{0.449}} &\scalebox{0.78}{0.526} &\scalebox{0.78}{0.516} &\scalebox{0.78}{0.450} &\scalebox{0.78}{0.459} \\ %&\scalebox{0.78}{4.431} &\scalebox{0.78}{1.729} \\
    \midrule
    
    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{ECL}}} 
    &  \scalebox{0.78}{96} & \textbf{\scalebox{0.78}{0.129}} & \textbf{\scalebox{0.78}{0.222}} & \scalebox{0.78}{0.148} & \scalebox{0.78}{0.240} & \textbf{\scalebox{0.78}{0.129}} & \textbf{\scalebox{0.78}{0.222}} & \scalebox{0.78}{0.219} & \scalebox{0.78}{0.314} & \scalebox{0.78}{0.137} & \scalebox{0.78}{0.238} &{\scalebox{0.78}{0.168}} &{\scalebox{0.78}{0.272}} &\scalebox{0.78}{0.140} &\scalebox{0.78}{0.237} & \scalebox{0.78}{0.247} & \scalebox{0.78}{0.345} &\scalebox{0.78}{0.193} &\scalebox{0.78}{0.308} &{\scalebox{0.78}{0.169}} &{\scalebox{0.78}{0.273}} &\scalebox{0.78}{0.201} &\scalebox{0.78}{0.317}  \\ %&\scalebox{0.78}{0.274} &\scalebox{0.78}{0.368} \\
    & \scalebox{0.78}{192} & \textbf{\scalebox{0.78}{0.143}} & \textbf{\scalebox{0.78}{0.235}} & \scalebox{0.78}{0.162} & {\scalebox{0.78}{0.253}} & \underline{\scalebox{0.78}{0.147}} & \underline{\scalebox{0.78}{0.240}} & \scalebox{0.78}{0.231} & \scalebox{0.78}{0.322} & \scalebox{0.78}{0.152} & \scalebox{0.78}{0.252} &{\scalebox{0.78}{0.184}} &\scalebox{0.78}{0.289} &\scalebox{0.78}{0.153} &{\scalebox{0.78}{0.249}} & \scalebox{0.78}{0.257} & \scalebox{0.78}{0.355} &\scalebox{0.78}{0.201} &\scalebox{0.78}{0.315} &{\scalebox{0.78}{0.182}} &\scalebox{0.78}{0.286} &\scalebox{0.78}{0.222} &\scalebox{0.78}{0.334} \\ %&\scalebox{0.78}{0.296} &\scalebox{0.78}{0.386} \\
    & \scalebox{0.78}{336} & \textbf{\scalebox{0.78}{0.152}} & \textbf{\scalebox{0.78}{0.248}} & \scalebox{0.78}{0.178} & {\scalebox{0.78}{0.269}} & \underline{\scalebox{0.78}{0.163}} & \underline{\scalebox{0.78}{0.259}} & \scalebox{0.78}{0.246} & \scalebox{0.78}{0.337} & \scalebox{0.78}{0.166} & \scalebox{0.78}{0.268} &{\scalebox{0.78}{0.198}} &{\scalebox{0.78}{0.300}} &\scalebox{0.78}{0.169} &{\scalebox{0.78}{0.267}} & \scalebox{0.78}{0.269} & \scalebox{0.78}{0.369} &\scalebox{0.78}{0.214} &\scalebox{0.78}{0.329} &{\scalebox{0.78}{0.200}} &\scalebox{0.78}{0.304} &\scalebox{0.78}{0.231} &\scalebox{0.78}{0.338}  \\ %&\scalebox{0.78}{0.300} &\scalebox{0.78}{0.394} \\
    & \scalebox{0.78}{720} & \textbf{\scalebox{0.78}{0.176}} & \textbf{\scalebox{0.78}{0.272}} & \scalebox{0.78}{0.225} & \scalebox{0.78}{0.317} & \underline{\scalebox{0.78}{0.197}} & \underline{\scalebox{0.78}{0.290}} & \scalebox{0.78}{0.280} & \scalebox{0.78}{0.363} & \scalebox{0.78}{0.201} & \scalebox{0.78}{0.302} &{\scalebox{0.78}{0.220}} &{\scalebox{0.78}{0.320}} &\scalebox{0.78}{0.203} &\scalebox{0.78}{0.301} & \scalebox{0.78}{0.299} & \scalebox{0.78}{0.390} &\scalebox{0.78}{0.246} &\scalebox{0.78}{0.355} &{\scalebox{0.78}{0.222}} &{\scalebox{0.78}{0.321}} &\scalebox{0.78}{0.254} &\scalebox{0.78}{0.361} \\ %&\scalebox{0.78}{0.373} &\scalebox{0.78}{0.439} \\
    \cmidrule(lr){2-24}
    & \scalebox{0.78}{Avg} & \textbf{\scalebox{0.78}{0.150}} & \textbf{\scalebox{0.78}{0.244}} & \scalebox{0.78}{0.178} & \scalebox{0.78}{0.270} & \underline{\scalebox{0.78}{0.159}} & \underline{\scalebox{0.78}{0.252}} & \scalebox{0.78}{0.244} & \scalebox{0.78}{0.334} & \scalebox{0.78}{0.164} & \scalebox{0.78}{0.265} &{\scalebox{0.78}{0.192}} &{\scalebox{0.78}{0.295}} &\scalebox{0.78}{0.166} &\scalebox{0.78}{0.263} & \scalebox{0.78}{0.268} & \scalebox{0.78}{0.365} &\scalebox{0.78}{0.214} &\scalebox{0.78}{0.327} &{\scalebox{0.78}{0.193}} &{\scalebox{0.78}{0.296}} &\scalebox{0.78}{0.227} &\scalebox{0.78}{0.338} \\ %&\scalebox{0.78}{0.311} &\scalebox{0.78}{0.397} \\
    \midrule

    % \multirow{5}{*}{\rotatebox{90}{\update{\scalebox{0.95}{Exchange}}}}
    % &  \scalebox{0.78}{96} & \boldres{\scalebox{0.78}{0.086}} & \secondres{\scalebox{0.78}{0.206}} & \scalebox{0.78}{0.093} & \scalebox{0.78}{0.217} & \secondres{\scalebox{0.78}{0.088}} & \boldres{\scalebox{0.78}{0.205}} & \scalebox{0.78}{0.256} & \scalebox{0.78}{0.367} & \scalebox{0.78}{0.094} & \scalebox{0.78}{0.218} & \scalebox{0.78}{0.107} & \scalebox{0.78}{0.234} & \scalebox{0.78}{0.088} & \scalebox{0.78}{0.218} & \scalebox{0.78}{0.267} & \scalebox{0.78}{0.396} & \scalebox{0.78}{0.148} & \scalebox{0.78}{0.278} & \scalebox{0.78}{0.111} & \scalebox{0.78}{0.237} & \scalebox{0.78}{0.197} & \scalebox{0.78}{0.323} \\ %& \scalebox{0.78}{0.847} & \scalebox{0.78}{0.752} \\
    % &  \scalebox{0.78}{192} & \scalebox{0.78}{0.177} & \secondres{\scalebox{0.78}{0.299}} & \scalebox{0.78}{0.184} & \scalebox{0.78}{0.307} & \boldres{\scalebox{0.78}{0.176}} & \boldres{\scalebox{0.78}{0.299}} & \scalebox{0.78}{0.470} & \scalebox{0.78}{0.509} & \scalebox{0.78}{0.184} & \scalebox{0.78}{0.307} & \scalebox{0.78}{0.226} & \scalebox{0.78}{0.344} & \secondres{\scalebox{0.78}{0.176}} & \scalebox{0.78}{0.315} & \scalebox{0.78}{0.351} & \scalebox{0.78}{0.459} & \scalebox{0.78}{0.271} & \scalebox{0.78}{0.315} & \scalebox{0.78}{0.219} & \scalebox{0.78}{0.335} & \scalebox{0.78}{0.300} & \scalebox{0.78}{0.369} \\ %& \scalebox{0.78}{1.204} & \scalebox{0.78}{0.895} \\
    % &  \scalebox{0.78}{336} & \scalebox{0.78}{0.331} & \secondres{\scalebox{0.78}{0.417}} & \scalebox{0.78}{0.351} & \scalebox{0.78}{0.432}& \boldres{\scalebox{0.78}{0.301}} & \boldres{\scalebox{0.78}{0.397}} & \scalebox{0.78}{1.268} & \scalebox{0.78}{0.883} & \scalebox{0.78}{0.349} & \scalebox{0.78}{0.431} & \scalebox{0.78}{0.367} & \scalebox{0.78}{0.448} & \secondres{\scalebox{0.78}{0.313}} & \scalebox{0.78}{0.427} & \scalebox{0.78}{1.324} & \scalebox{0.78}{0.853} & \scalebox{0.78}{0.460} & \scalebox{0.78}{0.427} & \scalebox{0.78}{0.421} & \scalebox{0.78}{0.476} & \scalebox{0.78}{0.509} & \scalebox{0.78}{0.524} \\ %& \scalebox{0.78}{1.672} & \scalebox{0.78}{1.036} \\
    % &  \scalebox{0.78}{720} & \secondres{\scalebox{0.78}{0.847}} & \boldres{\scalebox{0.78}{0.691}} & \scalebox{0.78}{0.886} & \scalebox{0.78}{0.714} & \scalebox{0.78}{0.901} & \scalebox{0.78}{0.714} & \scalebox{0.78}{1.767} & \scalebox{0.78}{1.068} & \scalebox{0.78}{0.852} & \scalebox{0.78}{0.698} & \scalebox{0.78}{0.964} & \scalebox{0.78}{0.746} & \boldres{\scalebox{0.78}{0.839}} & \scalebox{0.78}{0.695} & \scalebox{0.78}{1.058} & \scalebox{0.78}{0.797} & \scalebox{0.78}{1.195} & \secondres{\scalebox{0.78}{0.695}} & \scalebox{0.78}{1.092} & \scalebox{0.78}{0.769} & \scalebox{0.78}{1.447} & \scalebox{0.78}{0.941} \\ %& \scalebox{0.78}{2.478} & \scalebox{0.78}{1.310} \\
    % \cmidrule(lr){2-24}
    % &  \scalebox{0.78}{Avg} & \secondres{\scalebox{0.78}{0.360}} & \boldres{\scalebox{0.78}{0.403}} & \scalebox{0.78}{0.378} & \scalebox{0.78}{0.417} & \scalebox{0.78}{0.367} & \secondres{\scalebox{0.78}{0.404}} & \scalebox{0.78}{0.940} & \scalebox{0.78}{0.707} & \scalebox{0.78}{0.370} & \scalebox{0.78}{0.413} & \scalebox{0.78}{0.416} & \scalebox{0.78}{0.443} & \boldres{\scalebox{0.78}{0.354}} & \scalebox{0.78}{0.414} & \scalebox{0.78}{0.750} & \scalebox{0.78}{0.626} & \scalebox{0.78}{0.519} & \scalebox{0.78}{0.429} & \scalebox{0.78}{0.461} & \scalebox{0.78}{0.454} & \scalebox{0.78}{0.613} & \scalebox{0.78}{0.539} \\ %& \scalebox{0.78}{1.550} & \scalebox{0.78}{0.998} \\


    %\midrule
    
    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{Traffic}}} 
    & \scalebox{0.78}{96} & \textbf{\scalebox{0.78}{0.330}} & \textbf{\scalebox{0.78}{0.232}} & \scalebox{0.78}{0.395} & \scalebox{0.78}{0.268} & \underline{\scalebox{0.78}{0.360}} & \underline{\scalebox{0.78}{0.249}} & {\scalebox{0.78}{0.522}} & {\scalebox{0.78}{0.290}} & \scalebox{0.78}{0.390} & \scalebox{0.78}{0.275} &{\scalebox{0.78}{0.593}} &{\scalebox{0.78}{0.321}} &\scalebox{0.78}{0.410} &\scalebox{0.78}{0.282} & \scalebox{0.78}{0.788} & \scalebox{0.78}{0.499} &{\scalebox{0.78}{0.587}} &\scalebox{0.78}{0.366} &\scalebox{0.78}{0.612} &{\scalebox{0.78}{0.338}} &\scalebox{0.78}{0.613} &\scalebox{0.78}{0.388} \\ %&\scalebox{0.78}{0.719} &\scalebox{0.78}{0.391}\\
    & \scalebox{0.78}{192} & \textbf{\scalebox{0.78}{0.332}} & \textbf{\scalebox{0.78}{0.232}} & \scalebox{0.78}{0.417} & \scalebox{0.78}{0.276} & \underline{\scalebox{0.78}{0.379}} & \underline{\scalebox{0.78}{0.256}} & {\scalebox{0.78}{0.530}} & {\scalebox{0.78}{0.293}} & \scalebox{0.78}{0.402} & \scalebox{0.78}{0.278} &\scalebox{0.78}{0.617} &{\scalebox{0.78}{0.336}} &{\scalebox{0.78}{0.423}} &\scalebox{0.78}{0.287} & \scalebox{0.78}{0.789} & \scalebox{0.78}{0.505} &\scalebox{0.78}{0.604} &\scalebox{0.78}{0.373} &\scalebox{0.78}{0.613} &{\scalebox{0.78}{0.340}} &\scalebox{0.78}{0.616} &\scalebox{0.78}{0.382}  \\ %&\scalebox{0.78}{0.696} &\scalebox{0.78}{0.379} \\
    & \scalebox{0.78}{336} & \textbf{\scalebox{0.78}{0.342}} & \textbf{\scalebox{0.78}{0.236}} & \scalebox{0.78}{0.433} & \scalebox{0.78}{0.283} & \underline{\scalebox{0.78}{0.392}} & \underline{\scalebox{0.78}{0.264}} & \scalebox{0.78}{0.558} & {\scalebox{0.78}{0.305}}  & \scalebox{0.78}{0.415} & \scalebox{0.78}{0.288} &\scalebox{0.78}{0.629} &{\scalebox{0.78}{0.336}}  &{\scalebox{0.78}{0.436}} &\scalebox{0.78}{0.296} & \scalebox{0.78}{0.797} & \scalebox{0.78}{0.508}&\scalebox{0.78}{0.621} &\scalebox{0.78}{0.383} &\scalebox{0.78}{0.618} &{\scalebox{0.78}{0.328}} &\scalebox{0.78}{0.622} &\scalebox{0.78}{0.337} \\ %&\scalebox{0.78}{0.777} &\scalebox{0.78}{0.420} \\
    & \scalebox{0.78}{720} & \textbf{\scalebox{0.78}{0.365}} & \textbf{\scalebox{0.78}{0.244}} & \scalebox{0.78}{0.467} & \scalebox{0.78}{0.302} & \underline{\scalebox{0.78}{0.432}} & \underline{\scalebox{0.78}{0.286}} & \scalebox{0.78}{0.589} & {\scalebox{0.78}{0.328}}  & \scalebox{0.78}{0.449} & \scalebox{0.78}{0.307} &\scalebox{0.78}{0.640} &{\scalebox{0.78}{0.350}} &\scalebox{0.78}{0.466} &\scalebox{0.78}{0.315} & \scalebox{0.78}{0.841} & \scalebox{0.78}{0.523} &{\scalebox{0.78}{0.626}} &\scalebox{0.78}{0.382} &\scalebox{0.78}{0.653} &{\scalebox{0.78}{0.355}} &\scalebox{0.78}{0.660} &\scalebox{0.78}{0.408} \\ %&\scalebox{0.78}{0.864} &\scalebox{0.78}{0.472} \\
    \cmidrule(lr){2-24}
    & \scalebox{0.78}{Avg} & \textbf{\scalebox{0.78}{0.342}} & \textbf{\scalebox{0.78}{0.236}} & \scalebox{0.78}{0.428} & \scalebox{0.78}{0.282} & \underline{\scalebox{0.78}{0.390}} & \underline{\scalebox{0.78}{0.263}} & {\scalebox{0.78}{0.550}} & {\scalebox{0.78}{0.304}} & \scalebox{0.78}{0.414} & \scalebox{0.78}{0.287} &{\scalebox{0.78}{0.620}} &{\scalebox{0.78}{0.336}} &\scalebox{0.78}{0.433} &\scalebox{0.78}{0.295} & \scalebox{0.78}{0.804} & \scalebox{0.78}{0.509} &{\scalebox{0.78}{0.610}} &\scalebox{0.78}{0.376} &\scalebox{0.78}{0.624} &{\scalebox{0.78}{0.340}} &\scalebox{0.78}{0.628} &\scalebox{0.78}{0.379} \\ %&\scalebox{0.78}{0.764} &\scalebox{0.78}{0.416} \\
    \midrule
    
    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{Weather}}} 
    &  \scalebox{0.78}{96} & \underline{\scalebox{0.78}{0.157}} & \underline{\scalebox{0.78}{0.203}} & \scalebox{0.78}{0.174} & \scalebox{0.78}{0.214} & \textbf{\scalebox{0.78}{0.149}} & \textbf{\scalebox{0.78}{0.198}} & {\scalebox{0.78}{0.158}} & \scalebox{0.78}{0.230}  & \scalebox{0.78}{0.166} & \scalebox{0.78}{0.221} &{\scalebox{0.78}{0.172}} &{\scalebox{0.78}{0.220}} & \scalebox{0.78}{0.176} &\scalebox{0.78}{0.237} & \scalebox{0.78}{0.221} & \scalebox{0.78}{0.306} & \scalebox{0.78}{0.217} &\scalebox{0.78}{0.296} & {\scalebox{0.78}{0.173}} &{\scalebox{0.78}{0.223}} & \scalebox{0.78}{0.266} &\scalebox{0.78}{0.336} \\ %& \scalebox{0.78}{0.300} &\scalebox{0.78}{0.384}  \\
    & \scalebox{0.78}{192} & \underline{\scalebox{0.78}{0.200}} & \underline{\scalebox{0.78}{0.246}} & \scalebox{0.78}{0.221} & \scalebox{0.78}{0.254} & \textbf{\scalebox{0.78}{0.194}} & \textbf{\scalebox{0.78}{0.241}} & {\scalebox{0.78}{0.206}} & \scalebox{0.78}{0.277} & \scalebox{0.78}{0.207} & \scalebox{0.78}{0.261} &{\scalebox{0.78}{0.219}} &{\scalebox{0.78}{0.261}}  & \scalebox{0.78}{0.220} &\scalebox{0.78}{0.282} & \scalebox{0.78}{0.261} & \scalebox{0.78}{0.340} & \scalebox{0.78}{0.276} &\scalebox{0.78}{0.336} & \scalebox{0.78}{0.245} &\scalebox{0.78}{0.285} & \scalebox{0.78}{0.307} &\scalebox{0.78}{0.367} \\ %& \scalebox{0.78}{0.598} &\scalebox{0.78}{0.544} \\
    & \scalebox{0.78}{336} & \textbf{\scalebox{0.78}{0.241}} & \textbf{\scalebox{0.78}{0.281}} & \scalebox{0.78}{0.278} & \scalebox{0.78}{0.296} & \underline{\scalebox{0.78}{0.245}} & \underline{\scalebox{0.78}{0.282}} & {\scalebox{0.78}{0.272}} & \scalebox{0.78}{0.335} & \scalebox{0.78}{0.251} & \scalebox{0.78}{0.298} &{\scalebox{0.78}{0.280}} &{\scalebox{0.78}{0.306}} & \scalebox{0.78}{0.265} &\scalebox{0.78}{0.319} & \scalebox{0.78}{0.309} & \scalebox{0.78}{0.378} & \scalebox{0.78}{0.339} &\scalebox{0.78}{0.380} & \scalebox{0.78}{0.321} &\scalebox{0.78}{0.338} & \scalebox{0.78}{0.359} &\scalebox{0.78}{0.395}\\ % &\scalebox{0.78}{0.578} &\scalebox{0.78}{0.523} \\
    & \scalebox{0.78}{720} & \textbf{\scalebox{0.78}{0.291}} & \textbf{\scalebox{0.78}{0.324}} & \scalebox{0.78}{0.358} & \scalebox{0.78}{0.349} & \underline{\scalebox{0.78}{0.314}} & \underline{\scalebox{0.78}{0.334}} & \scalebox{0.78}{0.398} & \scalebox{0.78}{0.418} & {\scalebox{0.78}{0.301}} & \scalebox{0.78}{0.338} &\scalebox{0.78}{0.365} &{\scalebox{0.78}{0.359}} & {\scalebox{0.78}{0.323}} &{\scalebox{0.78}{0.362}} & \scalebox{0.78}{0.377} & \scalebox{0.78}{0.427} & \scalebox{0.78}{0.403} &\scalebox{0.78}{0.428} & \scalebox{0.78}{0.414} &\scalebox{0.78}{0.410} & \scalebox{0.78}{0.419} &\scalebox{0.78}{0.428} \\ %& \scalebox{0.78}{1.059} &\scalebox{0.78}{0.741} \\
    \cmidrule(lr){2-24}
    & \scalebox{0.78}{Avg} & \textbf{\scalebox{0.78}{0.222}} & \textbf{\scalebox{0.78}{0.263}} & \scalebox{0.78}{0.258} & \scalebox{0.78}{0.279} & \underline{\scalebox{0.78}{0.225}} & \underline{\scalebox{0.78}{0.263}} & \scalebox{0.78}{0.259} & \scalebox{0.78}{0.315} & \scalebox{0.78}{0.231} & \scalebox{0.78}{0.286} &{\scalebox{0.78}{0.259}} &{\scalebox{0.78}{0.287}} &\scalebox{0.78}{0.246} &\scalebox{0.78}{0.300} & \scalebox{0.78}{0.292} & \scalebox{0.78}{0.363} &\scalebox{0.78}{0.309} &\scalebox{0.78}{0.360} &\scalebox{0.78}{0.288} &\scalebox{0.78}{0.314} &\scalebox{0.78}{0.338} &\scalebox{0.78}{0.382} \\ %&\scalebox{0.78}{0.634} &\scalebox{0.78}{0.548} \\
    \midrule
    
    % \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{Solar-Energy}}} 
    % &  \scalebox{0.78}{96} &\boldres{\scalebox{0.78}{0.203}} &\boldres{\scalebox{0.78}{0.237}} & \scalebox{0.78}{0.322} & \scalebox{0.78}{0.339} & \secondres{\scalebox{0.78}{0.234}} & \secondres{\scalebox{0.78}{0.286}} &\scalebox{0.78}{0.310} &\scalebox{0.78}{0.331} &\scalebox{0.78}{0.312} &\scalebox{0.78}{0.399} &\scalebox{0.78}{0.250} &\scalebox{0.78}{0.292} &\scalebox{0.78}{0.290} &\scalebox{0.78}{0.378} &\scalebox{0.78}{0.237} &\scalebox{0.78}{0.344} &\scalebox{0.78}{0.242} &\scalebox{0.78}{0.342} &\scalebox{0.78}{0.215} &\scalebox{0.78}{0.249} &\scalebox{0.78}{0.884} &\scalebox{0.78}{0.711}\\ % &\scalebox{0.78}{0.236} &\secondres{\scalebox{0.78}{0.259}} \\
    % & \scalebox{0.78}{192} &\boldres{\scalebox{0.78}{0.233}} &\boldres{\scalebox{0.78}{0.261}} & \scalebox{0.78}{0.359} & \scalebox{0.78}{0.356}& \secondres{\scalebox{0.78}{0.267}} & \secondres{\scalebox{0.78}{0.310}} &\scalebox{0.78}{0.734} &\scalebox{0.78}{0.725} &\scalebox{0.78}{0.339} &\scalebox{0.78}{0.416} &\scalebox{0.78}{0.296} &\scalebox{0.78}{0.318} &\scalebox{0.78}{0.320} &\scalebox{0.78}{0.398} &\scalebox{0.78}{0.280} &\scalebox{0.78}{0.380} &\scalebox{0.78}{0.285} &\scalebox{0.78}{0.380} &\scalebox{0.78}{0.254} &\scalebox{0.78}{0.272} &\scalebox{0.78}{0.834} &\scalebox{0.78}{0.692} \\ %&\boldres{\scalebox{0.78}{0.217}} &\secondres{\scalebox{0.78}{0.269}} \\
    % & \scalebox{0.78}{336} &\boldres{\scalebox{0.78}{0.248}} &\boldres{\scalebox{0.78}{0.273}} & \scalebox{0.78}{0.397} & \scalebox{0.78}{0.369}& \secondres{\scalebox{0.78}{0.290}}  &\secondres{\scalebox{0.78}{0.315}} &\scalebox{0.78}{0.750} &\scalebox{0.78}{0.735} &\scalebox{0.78}{0.368} &\scalebox{0.78}{0.430} &\scalebox{0.78}{0.319} &\scalebox{0.78}{0.330} &\scalebox{0.78}{0.353} &\scalebox{0.78}{0.415} &\scalebox{0.78}{0.304} &\scalebox{0.78}{0.389} &\scalebox{0.78}{0.282} &\scalebox{0.78}{0.376} &\scalebox{0.78}{0.290} &\scalebox{0.78}{0.296} &\scalebox{0.78}{0.941} &\scalebox{0.78}{0.723} \\ %&\secondres{\scalebox{0.78}{0.249}} &\secondres{\scalebox{0.78}{0.283}}\\
    % & \scalebox{0.78}{720} &\boldres{\scalebox{0.78}{0.249}} &\boldres{\scalebox{0.78}{0.275}} & \scalebox{0.78}{0.397} & \scalebox{0.78}{0.356} & \secondres{\scalebox{0.78}{0.289}} &\secondres{\scalebox{0.78}{0.317}} &\scalebox{0.78}{0.769} &\scalebox{0.78}{0.765} &\scalebox{0.78}{0.370} &\scalebox{0.78}{0.425} &\scalebox{0.78}{0.338} &\scalebox{0.78}{0.337} &\scalebox{0.78}{0.356} &\scalebox{0.78}{0.413} &\scalebox{0.78}{0.308} &\scalebox{0.78}{0.388} &\scalebox{0.78}{0.357} &\scalebox{0.78}{0.427} &\scalebox{0.78}{0.285} &\scalebox{0.78}{0.295} &\scalebox{0.78}{0.882} &\scalebox{0.78}{0.717} \\ %&\boldres{\scalebox{0.78}{0.241}} &\boldres{\scalebox{0.78}{0.317}}\\
    % \cmidrule(lr){2-24}
    % & \scalebox{0.78}{Avg} &\boldres{\scalebox{0.78}{0.233}} &\boldres{\scalebox{0.78}{0.262}} & \scalebox{0.78}{0.369} & \scalebox{0.78}{0.356} &\secondres{\scalebox{0.78}{0.270}} &\secondres{\scalebox{0.78}{0.307}} &\scalebox{0.78}{0.641} &\scalebox{0.78}{0.639} &\scalebox{0.78}{0.347} &\scalebox{0.78}{0.417} &\scalebox{0.78}{0.301} &\scalebox{0.78}{0.319} &\scalebox{0.78}{0.330} &\scalebox{0.78}{0.401} &\scalebox{0.78}{0.282} &\scalebox{0.78}{0.375} &\scalebox{0.78}{0.291} &\scalebox{0.78}{0.381} &\scalebox{0.78}{0.261} &\scalebox{0.78}{0.381} &\scalebox{0.78}{0.885} &\scalebox{0.78}{0.711} \\ %&\secondres{\scalebox{0.78}{0.235}} &\secondres{\scalebox{0.78}{0.280}}\\
    % \midrule
      \multicolumn{2}{c|}{\scalebox{0.78}{{$1^{\text{st}}$ Count}}} & \scalebox{0.78}{{33}} & \scalebox{0.78}{{33}} & \scalebox{0.78}{0} & \scalebox{0.78}{{0}} & \scalebox{0.78}{{2}} & \scalebox{0.78}{2} & \scalebox{0.78}{0} & \scalebox{0.78}{0} & \scalebox{0.78}{0} & \scalebox{0.78}{0} & \scalebox{0.78}{0} & \scalebox{0.78}{0} & \scalebox{0.78}{0} & \scalebox{0.78}{0} & \scalebox{0.78}{0} & \scalebox{0.78}{0} & \scalebox{0.78}{0} & \scalebox{0.78}{0} & \scalebox{0.78}{0} & \scalebox{0.78}{0} & \scalebox{0.78}{0} & \scalebox{0.78}{0} \\ %& \scalebox{0.78}{2} & \scalebox{0.78}{1}\\
    \bottomrule
  \end{tabular}
    \end{small}
  \end{threeparttable}
%}
\label{tab:main_result}
\end{table*}
Comprehensive forecasting results are listed in Table~\ref{tab:main_result} with the best in \textbf{Bold} and the second \underline{underlined}. The lower MSE/MAE indicates the more accurate prediction result. Overall, PDETime achieves the best performance on most settings across seven real-world datasets compared with historical-value-based and time-index-based models. Additionally, experimental results also show that the performance of the proposed PDETime changes quite steadily as the prediction length $H$ increases. For instance, the MSE of PDETime increases from 0.330 to 0.365 on the Traffic dataset, while the MSE of PatchTST increases from 0.360 to 0.432, which is the SOTA historical-value-based model. This phenomenon was observed in other datasets and settings as well, indicating that PDETime retains better long-term robustness, which is meaningful for real-world practical applications. 



%The proposed \textcolor{blue}{xxx} achieves consistent state-of-the-art performance.

%\subsection{Ablation Study}
\begin{table*}[!]
\caption{Ablation study on variants of PDETime. -Temporal refers that removing the temporal domain feature $t_{\tau}$; -Spatial refers that removing the historical observations $x_{his}$; - Initial  refers that removing the initial condition $x_{\tau_{0}}$. The best results are highlighted in \textbf{bold}.}
    \centering
     \vskip -0.0in
    \vspace{3pt}
    \centering
    %\renewcommand{\arraystretch}{0.85} 
    \setlength{\tabcolsep}{3pt}
    \begin{threeparttable}
    \begin{small}
        
    \begin{tabular}{c|c|cc| cc|cc| cc|cc| ccc}
    \toprule
    \multirow{2}{*}{\scalebox{0.8}{Dataset}} & \scalebox{0.8}{Models} & \multicolumn{2}{c|}{\scalebox{0.8}{PDETime}} & \multicolumn{2}{c|}{\scalebox{0.8}{-Temporal}} & \multicolumn{2}{c|}{\scalebox{0.8}{-Spatial}} & \multicolumn{2}{c|}{\scalebox{0.8}{-Initial }} & \multicolumn{2}{c|}{\scalebox{0.9}{-Temporal -Spatial}}  & \multicolumn{2}{c}{\scalebox{0.9}{- All}} \\
    %\multicolumn{2}{c}{\scalebox{0.8}{His}} & \multicolumn{2}{c}{\scalebox{0.8}{His -Initial}} & \multicolumn{2}{c}{\scalebox{0.8}{His -Spatial}} & \multicolumn{2}{c}{\scalebox{0.8}{His -All}} \\
     & \scalebox{0.8}{Metric} & \scalebox{0.8}{MSE} & \scalebox{0.8}{MAE} & \scalebox{0.8}{MSE} & \scalebox{0.8}{MAE} & \scalebox{0.8}{MSE} & \scalebox{0.8}{MAE} & \scalebox{0.8}{MSE} & \scalebox{0.8}{MAE} & \scalebox{0.8}{MSE} & \scalebox{0.8}{MAE} & \scalebox{0.8}{MSE} & \scalebox{0.8}{MAE}  \\
     \midrule
     \multirow{4}{*}{\scalebox{0.9}{Traffic}} &\scalebox{0.8}{96} & \scalebox{0.8}{0.330} & \scalebox{0.8}{\textbf{0.232}} & \scalebox{0.8}{0.336} & \scalebox{0.8}{0.236} & \scalebox{0.8}{\textbf{0.329}} & \scalebox{0.8}{\textbf{0.232}} & \scalebox{0.8}{0.334} & \scalebox{0.8}{0.235} & \scalebox{0.8}{0.394} & \scalebox{0.8}{0.268} & \scalebox{0.8}{0.401} & \scalebox{0.8}{0.269}  \\
     &\scalebox{0.8}{192} & \scalebox{0.8}{\textbf{0.332}} & \scalebox{0.8}{\textbf{0.232}} & \scalebox{0.8}{0.368} & \scalebox{0.8}{0.247} & \scalebox{0.8}{0.336} & \scalebox{0.8}{0.234} & \scalebox{0.8}{0.334} & \scalebox{0.8}{\textbf{0.232}} & \scalebox{0.8}{0.407} & \scalebox{0.8}{0.269} & \scalebox{0.8}{0.413} & \scalebox{0.8}{0.270}  \\
     &\scalebox{0.8}{336} & \scalebox{0.8}{\textbf{0.342}} & \scalebox{0.8}{\textbf{0.236}} & \scalebox{0.8}{0.378} & \scalebox{0.8}{0.251} & \scalebox{0.8}{0.344} & \scalebox{0.8}{\textbf{0.236}} & \scalebox{0.8}{0.343} & \scalebox{0.8}{\textbf{0.236}} & \scalebox{0.8}{0.419} & \scalebox{0.8}{0.273} & \scalebox{0.8}{0.426} & \scalebox{0.8}{0.272}  \\
     &\scalebox{0.8}{720} & \scalebox{0.8}{\textbf{0.365}} & \scalebox{0.8}{\textbf{0.244}} & \scalebox{0.8}{0.406} & \scalebox{0.8}{0.265} & \scalebox{0.8}{0.371} & \scalebox{0.8}{0.250} & \scalebox{0.8}{0.368} & \scalebox{0.8}{0.250} & \scalebox{0.8}{0.453} & \scalebox{0.8}{0.291} & \scalebox{0.8}{0.671} & \scalebox{0.8}{0.406}  \\
     \midrule
     \multirow{4}{*}{\scalebox{0.9}{Weather}} &\scalebox{0.8}{96} & \scalebox{0.8}{\textbf{0.157}} & \scalebox{0.8}{\textbf{0.203}} & \scalebox{0.8}{0.158} & \scalebox{0.8}{0.205} & \scalebox{0.8}{0.159} & \scalebox{0.8}{0.205} & \scalebox{0.8}{0.169} & \scalebox{0.8}{0.213} & \scalebox{0.8}{0.159} & \scalebox{0.8}{0.205} & \scalebox{0.8}{0.166} & \scalebox{0.8}{0.212}  \\
     &\scalebox{0.8}{192} & \scalebox{0.8}{0.200} & \scalebox{0.8}{0.246} & \scalebox{0.8}{0.206} & \scalebox{0.8}{0.253} & \scalebox{0.8}{\textbf{0.198}} & \scalebox{0.8}{\textbf{0.243}} & \scalebox{0.8}{0.208} & \scalebox{0.8}{0.248} & \scalebox{0.8}{\textbf{0.198}} & \scalebox{0.8}{\textbf{0.243}} & \scalebox{0.8}{0.208} & \scalebox{0.8}{0.250}  \\
     &\scalebox{0.8}{336} & \scalebox{0.8}{0.241} & \scalebox{0.8}{0.281} & \scalebox{0.8}{\textbf{0.240}} & \scalebox{0.8}{0.278} & \scalebox{0.8}{0.246} & \scalebox{0.8}{0.282} & \scalebox{0.8}{0.245} & \scalebox{0.8}{0.287} & \scalebox{0.8}{\textbf{0.240}} & \scalebox{0.8}{\textbf{0.277}} & \scalebox{0.8}{0.244} & \scalebox{0.8}{0.283}  \\
     &\scalebox{0.8}{720} & \scalebox{0.8}{0.291} & \scalebox{0.8}{0.324} & \scalebox{0.8}{0.292} & \scalebox{0.8}{0.323} & \scalebox{0.8}{\textbf{0.290}} & \scalebox{0.8}{\textbf{0.322}} & \scalebox{0.8}{0.300} & \scalebox{0.8}{0.337} & \scalebox{0.8}{0.294} & \scalebox{0.8}{0.327} & \scalebox{0.8}{0.299} & \scalebox{0.8}{0.337}  \\
     \bottomrule
    \end{tabular}
    \end{small}
    \end{threeparttable}
    \label{tab:ablation}
\end{table*}
We perform ablation studies on the Traffic and Weather datasets to validate the effect of \textbf{temporal feature} $t_{\tau}$, \textbf{spatial feature} $x_{his}$ and \textbf{initial condition} $x_{\tau_{0}}$. The results are presented in Table~\ref{tab:ablation}. 
%We analyze the experimental results shown in Table~\ref{tab:ablation}.  
\textbf{1)} The initial condition $x_{t_{0}}$ is useful on most settings. As mentioned in Section~\ref{sec:approach}, we treat LMTF as Initial Value Problem, thus the effectiveness of $x_{\tau_{0}}$ validates the correctness of PDETime. 
%\textbf{2)} The effect of spatial features $x_{his}$ on PDETime is limited. This may be the feature of spatial domains $x$ is unknown, thus we utilize the historical observations $x_{his}$ to simulate $x$, but it may be not an effective way.
\textbf{2)} The impact of spatial features $x_{his}$ on PDETime is limited. This may be due to the fact that the true spatial domains $x$ are unknown, and we utilize the historical observations $x_{his}$ to simulate $x$. However, this approach may not be effective in capturing the true spatial features.
\textbf{3)} The influence of temporal feature $t_{\tau}$ on PDETime various significantly across different datasets. 
%Experimental results have shown that $x_{\tau}$ is of great helpful in Traffic dataset, but its effect on Weather is limited. 
Experimental results have shown that $t_{\tau}$ is highly beneficial in the Traffic dataset, but its effect on Weather dataset is limited. 
%We assume that the effect of $t_{\tau}$ on PDETime is related to the period of specific dataset. The period of Traffic may be one day or one week, so PDETime can easily learn the temporal feature of the dataset; on the contrary, the period of weather may be one year or longer, but this dataset only contains one year of data, thus PDETime cannot learn complete temporal feature.
For example, the period of Traffic dataset may be one day or one week, making it easier for PDETime to learn temporal features. On the other hand, the period of Weather dataset may be one year or longer, but the dataset only contains one year of data. As a result, PDETime cannot capture the complete temporal features in this case.
\par
We conduct an additional ablation study on Traffic to evaluate the ability of different INRs to extract features of $x_{his}$, $t_{\tau}$, and $\tau$. In this study, we compared the performance of using the GELU or Tanh activation function instead of sine in SIREN and making $\tau^{(0)}=[\text{GELU}(2\pi \textbf{B}_{1}\tau), \text{GELU}(2\pi \textbf{B}_{1}\tau),...]$ or $\tau^{(0)}=[\text{Tanh}(2\pi \textbf{B}_{1}\tau), \text{Tanh}(2\pi \textbf{B}_{1}\tau),...]$.
%in which GELU means using GELU instead of sine in SIREN and making $\tau^{(0)}=[\text{GELU}(2\pi \textbf{B}_{1}\tau), \text{GELU}(2\pi \textbf{B}_{1}\tau),...]$, and Tanh has the same form. 
Table~\ref{tab:act} presents the experimental results, we observe that the sine function (periodic functions) can extract features better than other non-decreasing activation functions. This is because the smooth, non-periodic activation functions fail to accurately model high-frequency information~\cite{sitzmann2020implicit}. Time series data is often periodic, and the periodic nature of the sine function makes it more effective in extracting time series features.
%and time series is often periodic~\cite{sitzmann2020implicit}. This makes non-periodic functions less effective in extracting time series features.
% This finding aligns with previous research~\cite{sitzmann2020implicit}, which suggests that non-periodic functions are less effective in capturing time series features. Therefore, the use of periodic activation functions, such as sine, can lead to better feature extraction in time series forecasting tasks.



\subsection{Effects of Hyper-parameters}
\begin{figure*}[!]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=0.92\textwidth-0.2in]{icml2024/figure/params.pdf}}\vspace{-5mm}
\caption{Evaluation on hyper-parameter impact. (a) MSE against hyper-parameter layers of INRs $k$ in Forecaster on ETTh1. (b) MSE against hyper-parameter layers of aggregation module $N$ in Forecaster on ETTh1. (c) MSE against hyper-parameter patch length $S$ in Estimator on ETTh1. }
\label{fig:params}
\end{center}\vspace{-11mm}
\end{figure*}
We evaluate the effect of four hyper-parameters: look-back window $L$, number of INRs layers $k$, number of aggregation layers $N$, and patch length $S$ on the ETTh1 and ETTh2 datasets. First, we perform a sensitivity on the look-back window $L=\mu \ast H$, where $H$ is the experimental setting. 
%The experimental results were shown in Table~\ref{tab:mu}, 
The results are presented in Table~\ref{tab:mu}. 
We observe that the test error decreases as $\mu$ increases, plateauing and even increasing slightly as $\mu$ grows extremely large when the horizon window is small. 
% In contrast, the test error increases as $\mu$ increases under a large horizon window. 
However, under a large horizon window, the test error increases as $\mu$ increases.
Next, we evaluate the hyper-parameters $N$ and $k$ on PDETime, as shown in Figure~\ref{fig:params} (a) and (b) respectively. We find that the performance of PDETime remains stable when $k \geq 3$. Additionally, the number of aggregation layers $N$ has a limited impact on PDETime.
%The impact of hyper-parameter $N$ and $k$ on PDETime are shown in Figure~\ref{fig:params} (a) and (b), respectively. We find that the performance of PDETime is stable when $k \geq 3$ and $N$ has limited impact on PDETime. The experimental results in Figure~\ref{fig:params} (c) demonstrate that the patch length $S$ has a large impace on PDETime. 
% In Figure~\ref{fig:params} (c), we prolong the patch length from 2 to 48 and evaluate MSE with different horizon windows. As $S$ increases, the prediction accuracy of PDETime first increases and then decreases and remains stable throughout. We further prolong the patch length to $S=H$, PDETime has the poor performance, which proves that error accumulation problem has a large impact on PDETime.
Furthermore, we investigate the effect of patch length $S$ on PDETime, as illustrated in Figure~\ref{fig:params} (c). We varied the patch length from 2 to 48 and evaluate MSE with different horizon windows. As the patch length $S$ increased, the prediction accuracy of PDETime initially improved, reached a peak, and then started to decline. However, the accuracy remains relatively stable throughout. We also extended the patch length to $S=H$. In this case, PDETime performed poorly, indicating that the accumulation of errors has a significant impact on the performance of PDETime.
Overall, these analyses provide insights into the effects of different hyper-parameters on the performance of PDETime and can guide the selection of appropriate settings for achieving optimal results.

% \subsection{Extra Experiments}
Due to space limitations, we put extra experiments on robustness and visualization experiments in  Appendix~\ref{sec:sup_results} and Appendix~\ref{sec:vis}, respectively.

    % \item Appendix~\ref{sec:exp_detail} provides details on the datasets and baselines.
    % \item Appendix~\ref{sec:sup_results} presents the results of the robustness experiments.
    % \item Appendix~\ref{sec:time_features} provides details of time features used in this work.
    % \item Appendix~\ref{sec:code} provides pseudocode of Encoder and Solver.
    % \item Appendix~\ref{sec:vis} visualizes the prediction results of PDETime on the Traffic dataset.


% \begin{figure*}[!]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\textwidth-0.2in]{icml2024/figure/params.pdf}}
% \caption{Evaluation on hyper-parameter impact. (a) MSE against hyper-parameter layers of INRs $k$ in Forecaster on ETTh1. (b) MSE against hyper-parameter layers of aggregation module $N$ in Forecaster on ETTh1. (c) MSE against hyper-parameter patch length $S$ in Estimator on ETTh1. }
% \label{fig:params}
% \end{center}
% \vskip -0.2in
% \end{figure*}




\begin{table}[!t]
\caption{Analysis on the look-back window length, based on the multiplier on horizon length, $L=\mu \ast H$. The best results are highlighted in \textbf{bold}.}
    \vskip -0.0in
    \vspace{3pt}
    \centering
    %\renewcommand{\arraystretch}{0.85} 
    \setlength{\tabcolsep}{3pt}
    \begin{threeparttable}  
    \begin{small}
        
    \begin{tabular}{cccccccccc}
    %\caption{Analysis on the look-back window length, based on the multiplier on horizon length, $L=\mu \ast H$. Best results are highlighted in \textbf{bold}.}
    \toprule
    \multirow{2}{*}{\scalebox{0.9}{Dataset}} & \scalebox{0.9}{Horizon} & \multicolumn{2}{c}{\scalebox{0.9}{96}} & \multicolumn{2}{c}{\scalebox{0.9}{192}} & \multicolumn{2}{c}{\scalebox{0.9}{336}} & \multicolumn{2}{c}{\scalebox{0.9}{720}} \\
      & \scalebox{0.9}{ $\mu$ } & \scalebox{0.8}{MSE} & \scalebox{0.8}{MAE} & \scalebox{0.8}{MSE} & \scalebox{0.8}{MAE} & \scalebox{0.8}{MSE} & \scalebox{0.8}{MAE} & \scalebox{0.8}{MSE} & \scalebox{0.8}{MAE} \\
     \midrule 
     \multirow{5}{*}{ETTh1} & \scalebox{0.9}{ 1 } & \scalebox{0.8}{0.378} & \scalebox{0.8}{0.386} & \scalebox{0.8}{0.415} & \scalebox{0.8}{0.411} & \scalebox{0.8}{\textbf{0.421}} & \scalebox{0.8}{\textbf{0.420}} & \scalebox{0.8}{\textbf{0.425}} & \scalebox{0.8}{\textbf{0.446}} \\
      & \scalebox{0.9}{ 3 } & \scalebox{0.8}{0.359} & \scalebox{0.8}{0.382} & \scalebox{0.8}{\textbf{0.394}} & \scalebox{0.8}{\textbf{0.404}} & \scalebox{0.8}{0.427} & \scalebox{0.8}{0.421} & \scalebox{0.8}{0.443} & \scalebox{0.8}{0.460} \\
      & \scalebox{0.9}{ 5 } & \scalebox{0.8}{0.360} & \scalebox{0.8}{0.385} & \scalebox{0.8}{0.396} & \scalebox{0.8}{0.405} & \scalebox{0.8}{\textbf{0.421}} & \scalebox{0.8}{\textbf{0.420}} & \scalebox{0.8}{0.495} & \scalebox{0.8}{0.501} \\
      & \scalebox{0.9}{ 7 } & \scalebox{0.8}{\textbf{0.354}} & \scalebox{0.8}{\textbf{0.381}} & \scalebox{0.8}{0.398} & \scalebox{0.8}{0.405} & \scalebox{0.8}{0.427} & \scalebox{0.8}{0.429} & \scalebox{0.8}{0.545} & \scalebox{0.8}{0.532} \\
      & \scalebox{0.9}{ 9 } & \scalebox{0.8}{0.356} & \scalebox{0.8}{\textbf{0.381}} & \scalebox{0.8}{0.397} & \scalebox{0.8}{0.406} & \scalebox{0.8}{0.446} & \scalebox{0.8}{0.440} & \scalebox{0.8}{1.220} & \scalebox{0.8}{0.882} \\
      \midrule
      \multirow{5}{*}{ETTh2} & \scalebox{0.9}{ 1 } & \scalebox{0.8}{0.288} & \scalebox{0.8}{0.335} & \scalebox{0.8}{0.357} & \scalebox{0.8}{0.381} & \scalebox{0.8}{0.380} & \scalebox{0.8}{0.404} & \scalebox{0.8}{\textbf{0.380}} & \scalebox{0.8}{\textbf{0.421}} \\
      & \scalebox{0.9}{ 3 } & \scalebox{0.8}{0.276} & \scalebox{0.8}{0.331} & \scalebox{0.8}{0.339} & \scalebox{0.8}{0.374} & \scalebox{0.8}{\textbf{0.358}} & \scalebox{0.8}{\textbf{0.395}} & \scalebox{0.8}{0.422} & \scalebox{0.8}{0.456} \\
      & \scalebox{0.9}{ 5 } & \scalebox{0.8}{0.275} & \scalebox{0.8}{0.333} & \scalebox{0.8}{\textbf{0.331}} & \scalebox{0.8}{\textbf{0.370}} & \scalebox{0.8}{0.360} & \scalebox{0.8}{0.408} & \scalebox{0.8}{0.622} & \scalebox{0.8}{0.576} \\
      & \scalebox{0.9}{ 7 } & \scalebox{0.8}{\textbf{0.268}} & \scalebox{0.8}{\textbf{0.330}} & \scalebox{0.8}{\textbf{0.331}} & \scalebox{0.8}{0.378} & \scalebox{0.8}{0.384} & \scalebox{0.8}{0.427} & \scalebox{0.8}{0.624} & \scalebox{0.8}{0.595} \\
      & \scalebox{0.9}{ 9 } & \scalebox{0.8}{0.272} & \scalebox{0.8}{0.331} & \scalebox{0.8}{\textbf{0.331}} & \scalebox{0.8}{0.378} & \scalebox{0.8}{0.412} & \scalebox{0.8}{0.451} & \scalebox{0.8}{0.797} & \scalebox{0.8}{0.689} \\
      \bottomrule
      
    \end{tabular}
    \end{small}
    \end{threeparttable}\vspace{-3mm}
    \label{tab:mu}
\end{table}


\begin{table}[t]
\caption{Analysis on INRs. PDETime refers to our proposed approach. GELU and Tanh refer to replacing SIREN and CFF with GELU or Tanh activation, respectively. The best results are highlighted in \textbf{bold}.}
    \vskip -0.0in
    \vspace{3pt}
    \centering
    %\renewcommand{\arraystretch}{0.85} 
    \setlength{\tabcolsep}{3.5pt}
    \begin{threeparttable}  
    \begin{small}
        
    \begin{tabular}{cccccccc}
    %\caption{Analysis on the look-back window length, based on the multiplier on horizon length, $L=\mu \ast H$. Best results are highlighted in \textbf{bold}.}
    \toprule
    \multirow{2}{*}{\scalebox{1.0}{Dataset}} & \scalebox{1.0}{Method} & \multicolumn{2}{c}{\scalebox{1.0}{PDETime}} & \multicolumn{2}{c}{\scalebox{1.0}{GELU}} & \multicolumn{2}{c}{\scalebox{1.0}{Tanh}} \\
      & \scalebox{1.0}{ Metric } & \scalebox{1.0}{MSE} & \scalebox{1.0}{MAE} & \scalebox{1.0}{MSE} & \scalebox{1.0}{MAE} & \scalebox{1.0}{MSE} & \scalebox{1.0}{MAE}  \\
     \midrule 
     \multirow{4}{*}{Traffic} & \scalebox{1.0}{ 96 } & \scalebox{1.0}{\textbf{0.330}} & \scalebox{1.0}{\textbf{0.232}} & \scalebox{1.0}{0.332} & \scalebox{1.0}{0.237} & \scalebox{1.0}{{0.338}} & \scalebox{1.0}{{0.233}} \\
      & \scalebox{1.0}{ 192 } & \scalebox{1.0}{\textbf{0.332}} & \scalebox{1.0}{\textbf{0.232}} & \scalebox{1.0}{{0.338}} & \scalebox{1.0}{{0.241}} & \scalebox{1.0}{0.339} & \scalebox{1.0}{0.235} \\
      & \scalebox{1.0}{ 336 } & \scalebox{1.0}{\textbf{0.342}} & \scalebox{1.0}{\textbf{0.236}} & \scalebox{1.0}{0.348} & \scalebox{1.0}{0.244} & \scalebox{1.0}{{0.348}} & \scalebox{1.0}{{0.238}}  \\
      & \scalebox{1.0}{ 720 } & \scalebox{1.0}{\textbf{0.365}} & \scalebox{1.0}{\textbf{0.244}} & \scalebox{1.0}{0.376} & \scalebox{1.0}{0.252} & \scalebox{1.0}{0.366} & \scalebox{1.0}{\textbf{0.244}} \\
      % \midrule
      % \multirow{4}{*}{Traffic} & \scalebox{1.0}{ 96 } & \scalebox{1.0}{\textbf{0.330}} & \scalebox{1.0}{\textbf{0.232}} & \scalebox{1.0}{0.332} & \scalebox{1.0}{0.237} & \scalebox{1.0}{{0.338}} & \scalebox{1.0}{{0.233}} \\
      % & \scalebox{1.0}{ 192 } & \scalebox{1.0}{\textbf{0.332}} & \scalebox{1.0}{\textbf{0.232}} & \scalebox{1.0}{{0.338}} & \scalebox{1.0}{{0.241}} & \scalebox{1.0}{0.339} & \scalebox{1.0}{0.235} \\
      % & \scalebox{1.0}{ 336 } & \scalebox{1.0}{\textbf{0.342}} & \scalebox{1.0}{\textbf{0.236}} & \scalebox{1.0}{0.348} & \scalebox{1.0}{0.244} & \scalebox{1.0}{{0.348}} & \scalebox{1.0}{{0.238}}  \\
      % & \scalebox{1.0}{ 720 } & \scalebox{1.0}{\textbf{0.365}} & \scalebox{1.0}{\textbf{0.244}} & \scalebox{1.0}{0.376} & \scalebox{1.0}{0.252} & \scalebox{1.0}{0.366} & \scalebox{1.0}{\textbf{0.244}} \\
      \bottomrule
      
    \end{tabular}
    \end{small}
    \end{threeparttable}\vspace{-3mm}
    \label{tab:act}
\end{table}



% \begin{table*}[h]
%   \caption{\update{Full results of the long-term forecasting task}. We compare extensive competitive models under different prediction lengths following the setting of TimesNet~\citeyearpar{wu2022timesnet}. The input sequence length is set to 336 and 512 for DLinear and PatchTST, and 96 for other historical-value-based baselines. \emph{Avg} means the average results from all four prediction lengths.}\label{tab:full_baseline_results}
%   \vskip -0.0in
%   \vspace{3pt}
%   \renewcommand{\arraystretch}{0.85} 
%   \centering
%   %\resizebox{1\columnwidth}{!}{
%   \begin{threeparttable}
%   \begin{small}
%   \renewcommand{\multirowsetup}{\centering}
%   \setlength{\tabcolsep}{2.5pt}
%   \begin{tabular}{c|c|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc}
%     \toprule
%     \multicolumn{2}{c}{\multirow{2}{*}{Models}} & 
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{\textbf{PDETime}}}} &
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{{iTransformer}}}} &
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{{PatchTST}}}} &
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Crossformer}}}  &
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{{DeepTime}}}} &
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{{TimesNet}}}} &
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{{DLinear}}}}&
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{SCINet}}} &
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{FEDformer}}} &
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Stationary}}} &
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Autoformer}}} \\
%     %&\multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Informer}}} 
%     \multicolumn{2}{c}{} &
%     \multicolumn{2}{c}{\scalebox{0.8}{\textbf{(Ours)}}} & 
%     \multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{liu2023itransformer}}} & 
%     \multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{nie2022time}}} & 
%     \multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{zhang2022crossformer}}}  & 
%     \multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{woo2023learning}}} & 
%     \multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{wu2022timesnet}}} & 
%     \multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{zeng2023transformers}}}& 
%     \multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{liu2022scinet}}} &
%     \multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{zhou2022fedformer}}} &
%     \multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{liu2022non}}} &
%     \multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{wu2021autoformer}}} \\
%     %&\multicolumn{2}{c}{\scalebox{0.8}{\citeyearpar{Informer}}} 
%     \cmidrule(lr){3-4} \cmidrule(lr){5-6}\cmidrule(lr){7-8} \cmidrule(lr){9-10}\cmidrule(lr){11-12}\cmidrule(lr){13-14} \cmidrule(lr){15-16} \cmidrule(lr){17-18} \cmidrule(lr){19-20} \cmidrule(lr){21-22} \cmidrule(lr){23-24}
%     \multicolumn{2}{c}{Metric}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} \\
%     \toprule
    
%     \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{ETTm1}}}
%     &  \scalebox{0.78}{96} & {\scalebox{0.78}{0.334}} & {\scalebox{0.78}{0.368}} & \scalebox{0.78}{0.355} & \scalebox{0.78}{0.376} & {\scalebox{0.78}{0.329}} & {\scalebox{0.78}{0.367}} & \scalebox{0.78}{0.404} & \scalebox{0.78}{0.426} & \scalebox{0.78}{0.672} & \scalebox{0.78}{0.571} &{\scalebox{0.78}{0.338}} &{\scalebox{0.78}{0.375}} &{\scalebox{0.78}{0.345}} &{\scalebox{0.78}{0.372}} & \scalebox{0.78}{0.418} & \scalebox{0.78}{0.438} &\scalebox{0.78}{0.379} &\scalebox{0.78}{0.419} &\scalebox{0.78}{0.386} &\scalebox{0.78}{0.398} &\scalebox{0.78}{0.505} &\scalebox{0.78}{0.475} \\ %&\scalebox{0.78}{0.672} &\scalebox{0.78}{0.571} \\
%     & \scalebox{0.78}{192} & \scalebox{0.78}{0.377} & \scalebox{0.78}{0.391} & \scalebox{0.78}{0.391} & \scalebox{0.78}{0.392} & {\scalebox{0.78}{0.367}} & {\scalebox{0.78}{0.385}} & \scalebox{0.78}{0.450} & \scalebox{0.78}{0.451} &\scalebox{0.78}{0.795} & \scalebox{0.78}{0.669} &{\scalebox{0.78}{0.374}} &{\scalebox{0.78}{0.387}}  &{\scalebox{0.78}{0.380}} &{\scalebox{0.78}{0.389}} & \scalebox{0.78}{0.439} & \scalebox{0.78}{0.450}  &\scalebox{0.78}{0.426} &\scalebox{0.78}{0.441} &\scalebox{0.78}{0.459} &\scalebox{0.78}{0.444} &\scalebox{0.78}{0.553} &\scalebox{0.78}{0.496} \\ %&\scalebox{0.78}{0.795} &\scalebox{0.78}{0.669}\\
%     & \scalebox{0.78}{336} & \scalebox{0.78}{0.426} & \scalebox{0.78}{0.420} & \scalebox{0.78}{0.424} & \scalebox{0.78}{0.415} & {\scalebox{0.78}{0.399}} & {\scalebox{0.78}{0.410}} & \scalebox{0.78}{0.532}  &\scalebox{0.78}{0.515} & \scalebox{0.78}{1.212} & \scalebox{0.78}{0.871} &{\scalebox{0.78}{0.410}} &{\scalebox{0.78}{0.411}}  &{\scalebox{0.78}{0.413}} &{\scalebox{0.78}{0.413}} & \scalebox{0.78}{0.490} & \scalebox{0.78}{0.485}  &\scalebox{0.78}{0.445} &\scalebox{0.78}{0.459} &\scalebox{0.78}{0.495} &\scalebox{0.78}{0.464} &\scalebox{0.78}{0.621} &\scalebox{0.78}{0.537} \\ %&\scalebox{0.78}{1.212} &\scalebox{0.78}{0.871} \\
%     & \scalebox{0.78}{720} & \scalebox{0.78}{0.491} & \scalebox{0.78}{0.459} & \scalebox{0.78}{0.487} & \scalebox{0.78}{0.450} & {\scalebox{0.78}{0.454}} & {\scalebox{0.78}{0.439}} & \scalebox{0.78}{0.666} & \scalebox{0.78}{0.589} & \scalebox{0.78}{1.166} & \scalebox{0.78}{0.823} &{\scalebox{0.78}{0.478}} &{\scalebox{0.78}{0.450}} &{\scalebox{0.78}{0.474}} &{\scalebox{0.78}{0.453}} & \scalebox{0.78}{0.595} & \scalebox{0.78}{0.550}  &\scalebox{0.78}{0.543} &\scalebox{0.78}{0.490} &\scalebox{0.78}{0.585} &\scalebox{0.78}{0.516} &\scalebox{0.78}{0.671} &\scalebox{0.78}{0.561} \\ %&\scalebox{0.78}{1.166} &\scalebox{0.78}{0.823} \\
%     \cmidrule(lr){2-24}
%     & \scalebox{0.78}{Avg} & \scalebox{0.78}{0.407} & \scalebox{0.78}{0.410} & \scalebox{0.78}{0.414} & \scalebox{0.78}{0.407} & {\scalebox{0.78}{0.387}} & {\scalebox{0.78}{0.400}} & \scalebox{0.78}{0.513} & \scalebox{0.78}{0.496} & \scalebox{0.78}{0.419} & \scalebox{0.78}{0.419} &{\scalebox{0.78}{0.400}} &{\scalebox{0.78}{0.406}}  &{\scalebox{0.78}{0.403}} &{\scalebox{0.78}{0.407}} & \scalebox{0.78}{0.485} & \scalebox{0.78}{0.481}  &\scalebox{0.78}{0.448} &\scalebox{0.78}{0.452} &\scalebox{0.78}{0.481} &\scalebox{0.78}{0.456} &\scalebox{0.78}{0.588} &\scalebox{0.78}{0.517} \\ %&\scalebox{0.78}{0.961} &\scalebox{0.78}{0.734} \\
%     \midrule
    
%     \multirow{5}{*}{\update{\rotatebox{90}{\scalebox{0.95}{ETTm2}}}}
%     &  \scalebox{0.78}{96} & {\scalebox{0.78}{0.180}} & {\scalebox{0.78}{0.264}} & \scalebox{0.78}{0.182} & \scalebox{0.78}{0.265} & {\scalebox{0.78}{0.175}} & {\scalebox{0.78}{0.259}} & \scalebox{0.78}{0.287} & \scalebox{0.78}{0.366} & \scalebox{0.78}{0.207} & \scalebox{0.78}{0.305} &{\scalebox{0.78}{0.187}} &\scalebox{0.78}{0.267} &\scalebox{0.78}{0.193} &\scalebox{0.78}{0.292} & \scalebox{0.78}{0.286} & \scalebox{0.78}{0.377} &\scalebox{0.78}{0.203} &\scalebox{0.78}{0.287} &{\scalebox{0.78}{0.192}} &\scalebox{0.78}{0.274} &\scalebox{0.78}{0.255} &\scalebox{0.78}{0.339} \\ % &\scalebox{0.78}{0.365} &\scalebox{0.78}{0.453} \\
%     & \scalebox{0.78}{192} & \scalebox{0.78}{0.250} & {\scalebox{0.78}{0.309}} & {\scalebox{0.78}{0.246}} & {\scalebox{0.78}{0.304}} & {\scalebox{0.78}{0.241}} & {\scalebox{0.78}{0.302}} & \scalebox{0.78}{0.414} & \scalebox{0.78}{0.492} & \scalebox{0.78}{0.290} & \scalebox{0.78}{0.364} &{\scalebox{0.78}{0.249}} &{\scalebox{0.78}{0.309}} &\scalebox{0.78}{0.284} &\scalebox{0.78}{0.362} & \scalebox{0.78}{0.399} & \scalebox{0.78}{0.445} &\scalebox{0.78}{0.269} &\scalebox{0.78}{0.328} &\scalebox{0.78}{0.280} &\scalebox{0.78}{0.339} &\scalebox{0.78}{0.281} &\scalebox{0.78}{0.340} \\ %&\scalebox{0.78}{0.533} &\scalebox{0.78}{0.563} \\
%     & \scalebox{0.78}{336} & {\scalebox{0.78}{0.311}} & {\scalebox{0.78}{0.348}} & \secondres{\scalebox{0.78}{0.307}} & \boldres{\scalebox{0.78}{0.342}} & \boldres{\scalebox{0.78}{0.305}} & \secondres{\scalebox{0.78}{0.343}}  & \scalebox{0.78}{0.597} & \scalebox{0.78}{0.542}  & \scalebox{0.78}{0.377} & \scalebox{0.78}{0.422} &{\scalebox{0.78}{0.321}} &{\scalebox{0.78}{0.351}} &\scalebox{0.78}{0.369} &\scalebox{0.78}{0.427} & \scalebox{0.78}{0.637} & \scalebox{0.78}{0.591} &\scalebox{0.78}{0.325} &\scalebox{0.78}{0.366} &\scalebox{0.78}{0.334} &\scalebox{0.78}{0.361} &\scalebox{0.78}{0.339} &\scalebox{0.78}{0.372} \\ %&\scalebox{0.78}{1.363} &\scalebox{0.78}{0.887} \\
%     & \scalebox{0.78}{720} & \scalebox{0.78}{0.412} & \scalebox{0.78}{0.407} & \secondres{\scalebox{0.78}{0.407}} & \boldres{\scalebox{0.78}{0.398}} & \boldres{\scalebox{0.78}{0.402}} & \secondres{\scalebox{0.78}{0.400}} & \scalebox{0.78}{1.730} & \scalebox{0.78}{1.042} & \scalebox{0.78}{0.558} & \scalebox{0.78}{0.524} &{\scalebox{0.78}{0.408}} &{\scalebox{0.78}{0.403}} &\scalebox{0.78}{0.554} &\scalebox{0.78}{0.522} & \scalebox{0.78}{0.960} & \scalebox{0.78}{0.735} &\scalebox{0.78}{0.421} &\scalebox{0.78}{0.415} &\scalebox{0.78}{0.417} &\scalebox{0.78}{0.413} &\scalebox{0.78}{0.433} &\scalebox{0.78}{0.432} \\ %&\scalebox{0.78}{3.379} &\scalebox{0.78}{1.338} \\
%     \cmidrule(lr){2-24}
%     & \scalebox{0.78}{Avg} & {\scalebox{0.78}{0.288}} & {\scalebox{0.78}{0.332}} & \secondres{\scalebox{0.78}{0.286}} & \secondres{\scalebox{0.78}{0.327}} & \boldres{\scalebox{0.78}{0.281}} & \boldres{\scalebox{0.78}{0.326}} & \scalebox{0.78}{0.757} & \scalebox{0.78}{0.610} & \scalebox{0.78}{0.358} & \scalebox{0.78}{0.404} &{\scalebox{0.78}{0.291}} &{\scalebox{0.78}{0.333}} &\scalebox{0.78}{0.350} &\scalebox{0.78}{0.401} & \scalebox{0.78}{0.571} & \scalebox{0.78}{0.537} &\scalebox{0.78}{0.305} &\scalebox{0.78}{0.349} &\scalebox{0.78}{0.306} &\scalebox{0.78}{0.347} &\scalebox{0.78}{0.327} &\scalebox{0.78}{0.371} \\ %&\scalebox{0.78}{1.410} &\scalebox{0.78}{0.810} \\
%     \midrule
    
%     \multirow{5}{*}{\rotatebox{90}{\update{\scalebox{0.95}{ETTh1}}}}
%     &  \scalebox{0.78}{96} & {\scalebox{0.78}{0.386}} & {\scalebox{0.78}{0.405}} & \scalebox{0.78}{0.386} & \boldres{\scalebox{0.78}{0.395}} & \scalebox{0.78}{0.414} & \scalebox{0.78}{0.419} & \scalebox{0.78}{0.423} & \scalebox{0.78}{0.448} & \scalebox{0.78}{0.479}& \scalebox{0.78}{0.464}  &\secondres{\scalebox{0.78}{0.384}} &{\scalebox{0.78}{0.402}} & \scalebox{0.78}{0.386} &\secondres{\scalebox{0.78}{0.400}} & \scalebox{0.78}{0.654} & \scalebox{0.78}{0.599} &\boldres{\scalebox{0.78}{0.376}} &\scalebox{0.78}{0.419} &\scalebox{0.78}{0.513} &\scalebox{0.78}{0.491} &\scalebox{0.78}{0.449} &\scalebox{0.78}{0.459}  \\ %&\scalebox{0.78}{0.865} &\scalebox{0.78}{0.713} \\
%     & \scalebox{0.78}{192} & \scalebox{0.78}{0.441} & \scalebox{0.78}{0.436} & {\scalebox{0.78}{0.437}} & \boldres{\scalebox{0.78}{0.424}} & \scalebox{0.78}{0.460} & \scalebox{0.78}{0.445} & \scalebox{0.78}{0.471} & \scalebox{0.78}{0.474}  & \scalebox{0.78}{0.525} & \scalebox{0.78}{0.492} &\secondres{\scalebox{0.78}{0.436}} &\secondres{\scalebox{0.78}{0.429}}  &{\scalebox{0.78}{0.437}} &{\scalebox{0.78}{0.432}} & \scalebox{0.78}{0.719} & \scalebox{0.78}{0.631} &\boldres{\scalebox{0.78}{0.420}} &\scalebox{0.78}{0.448} &\scalebox{0.78}{0.534} &\scalebox{0.78}{0.504} &\scalebox{0.78}{0.500} &\scalebox{0.78}{0.482} \\ %&\scalebox{0.78}{1.008} &\scalebox{0.78}{0.792} \\
%     & \scalebox{0.78}{336} & {\scalebox{0.78}{0.487}} & \secondres{\scalebox{0.78}{0.458}} & \secondres{\scalebox{0.78}{0.479}} & \boldres{\scalebox{0.78}{0.446}} & \scalebox{0.78}{0.501} & \scalebox{0.78}{0.466} & \scalebox{0.78}{0.570} & \scalebox{0.78}{0.546} & \scalebox{0.78}{0.565} & \scalebox{0.78}{0.515} &\scalebox{0.78}{0.491} &\scalebox{0.78}{0.469} &{\scalebox{0.78}{0.481}} & {\scalebox{0.78}{0.459}} & \scalebox{0.78}{0.778} & \scalebox{0.78}{0.659} &\boldres{\scalebox{0.78}{0.459}} &{\scalebox{0.78}{0.465}} &\scalebox{0.78}{0.588} &\scalebox{0.78}{0.535} &\scalebox{0.78}{0.521} &\scalebox{0.78}{0.496} \\ %&\scalebox{0.78}{1.107} &\scalebox{0.78}{0.809} \\
%     & \scalebox{0.78}{720} & {\scalebox{0.78}{0.503}} & {\scalebox{0.78}{0.491}} & \boldres{\scalebox{0.78}{0.481}} & 
%     \boldres{\scalebox{0.78}{0.470}} & \secondres{\scalebox{0.78}{0.500}} & \secondres{\scalebox{0.78}{0.488}} & \scalebox{0.78}{0.653} & \scalebox{0.78}{0.621} & \scalebox{0.78}{0.594} & \scalebox{0.78}{0.558} &\scalebox{0.78}{0.521} &{\scalebox{0.78}{0.500}} &\scalebox{0.78}{0.519} &\scalebox{0.78}{0.516} & \scalebox{0.78}{0.836} & \scalebox{0.78}{0.699} &{\scalebox{0.78}{0.506}} &{\scalebox{0.78}{0.507}} &\scalebox{0.78}{0.643} &\scalebox{0.78}{0.616} &{\scalebox{0.78}{0.514}} &\scalebox{0.78}{0.512}  \\ %&\scalebox{0.78}{1.181} &\scalebox{0.78}{0.865} \\
%     \cmidrule(lr){2-24}
%     & \scalebox{0.78}{Avg} & {\scalebox{0.78}{0.454}} & \secondres{\scalebox{0.78}{0.447}} & \secondres{\scalebox{0.78}{0.446}} & \boldres{\scalebox{0.78}{0.434}} & \scalebox{0.78}{0.469} & \scalebox{0.78}{0.454} & \scalebox{0.78}{0.529} & \scalebox{0.78}{0.522} & \scalebox{0.78}{0.541} & \scalebox{0.78}{0.507} &\scalebox{0.78}{0.458} &{\scalebox{0.78}{0.450}} &{\scalebox{0.78}{0.456}} &{\scalebox{0.78}{0.452}} & \scalebox{0.78}{0.747} & \scalebox{0.78}{0.647} &\boldres{\scalebox{0.78}{0.440}} &\scalebox{0.78}{0.460} &\scalebox{0.78}{0.570} &\scalebox{0.78}{0.537} &\scalebox{0.78}{0.496} &\scalebox{0.78}{0.487}  \\ %&\scalebox{0.78}{1.040} &\scalebox{0.78}{0.795} \\
%     \midrule

%     \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{ETTh2}}}
%     &  \scalebox{0.78}{96} & \secondres{\scalebox{0.78}{0.297}} & {\scalebox{0.78}{0.349}} & \boldres{\scalebox{0.78}{0.288}} & \boldres{\scalebox{0.78}{0.338}} & {\scalebox{0.78}{0.302}} & \secondres{\scalebox{0.78}{0.348}} & \scalebox{0.78}{0.745} & \scalebox{0.78}{0.584} &\scalebox{0.78}{0.400} & \scalebox{0.78}{0.440}  & {\scalebox{0.78}{0.340}} & {\scalebox{0.78}{0.374}} &{\scalebox{0.78}{0.333}} &{\scalebox{0.78}{0.387}} & \scalebox{0.78}{0.707} & \scalebox{0.78}{0.621}  &\scalebox{0.78}{0.358} &\scalebox{0.78}{0.397} &\scalebox{0.78}{0.476} &\scalebox{0.78}{0.458} &\scalebox{0.78}{0.346} &\scalebox{0.78}{0.388} \\ %&\scalebox{0.78}{3.755} &\scalebox{0.78}{1.525} \\
%     & \scalebox{0.78}{192} & \secondres{\scalebox{0.78}{0.380}} & \secondres{\scalebox{0.78}{0.400}} & \boldres{\scalebox{0.78}{0.374}} & \boldres{\scalebox{0.78}{0.390}} &{\scalebox{0.78}{0.388}} & {\scalebox{0.78}{0.400}} & \scalebox{0.78}{0.877} & \scalebox{0.78}{0.656} & \scalebox{0.78}{0.528} & \scalebox{0.78}{0.509} & {\scalebox{0.78}{0.402}} & {\scalebox{0.78}{0.414}} &\scalebox{0.78}{0.477} &\scalebox{0.78}{0.476} & \scalebox{0.78}{0.860} & \scalebox{0.78}{0.689} &{\scalebox{0.78}{0.429}} &{\scalebox{0.78}{0.439}} &\scalebox{0.78}{0.512} &\scalebox{0.78}{0.493} &\scalebox{0.78}{0.456} &\scalebox{0.78}{0.452} \\ %&\scalebox{0.78}{5.602} &\scalebox{0.78}{1.931} \\
%     & \scalebox{0.78}{336} & {\scalebox{0.78}{0.428}} & \secondres{\scalebox{0.78}{0.432}} & \boldres{\scalebox{0.78}{0.415}} & \boldres{\scalebox{0.78}{0.426}} & \secondres{\scalebox{0.78}{0.426}} & {\scalebox{0.78}{0.433}}& \scalebox{0.78}{1.043} & \scalebox{0.78}{0.731} & \scalebox{0.78}{0.643} & \scalebox{0.78}{0.571}  & {\scalebox{0.78}{0.452}} & {\scalebox{0.78}{0.452}} &\scalebox{0.78}{0.594} &\scalebox{0.78}{0.541} & \scalebox{0.78}{1.000} &\scalebox{0.78}{0.744} &\scalebox{0.78}{0.496} &\scalebox{0.78}{0.487} &\scalebox{0.78}{0.552} &\scalebox{0.78}{0.551} &{\scalebox{0.78}{0.482}} &\scalebox{0.78}{0.486}\\ % &\scalebox{0.78}{4.721} &\scalebox{0.78}{1.835} \\
%     & \scalebox{0.78}{720} & \secondres{\scalebox{0.78}{0.427}} & \secondres{\scalebox{0.78}{0.445}} & \boldres{\scalebox{0.78}{0.420}} & \boldres{\scalebox{0.78}{0.440}} & {\scalebox{0.78}{0.431}} & {\scalebox{0.78}{0.446}} & \scalebox{0.78}{1.104} & \scalebox{0.78}{0.763} & \scalebox{0.78}{0.874} & \scalebox{0.78}{0.679} & {\scalebox{0.78}{0.462}} & {\scalebox{0.78}{0.468}} &\scalebox{0.78}{0.831} &\scalebox{0.78}{0.657} & \scalebox{0.78}{1.249} & \scalebox{0.78}{0.838} &{\scalebox{0.78}{0.463}} &{\scalebox{0.78}{0.474}} &\scalebox{0.78}{0.562} &\scalebox{0.78}{0.560} &\scalebox{0.78}{0.515} &\scalebox{0.78}{0.511} \\ %&\scalebox{0.78}{3.647} &\scalebox{0.78}{1.625} \\
%     \cmidrule(lr){2-24}
%     & \scalebox{0.78}{Avg} & \secondres{\scalebox{0.78}{0.383}} & \secondres{\scalebox{0.78}{0.407}} & \boldres{\scalebox{0.78}{0.374}} & \boldres{\scalebox{0.78}{0.398}} & {\scalebox{0.78}{0.387}} & {\scalebox{0.78}{0.407}} & \scalebox{0.78}{0.942} & \scalebox{0.78}{0.684} & \scalebox{0.78}{0.611} & \scalebox{0.78}{0.550}  &{\scalebox{0.78}{0.414}} &{\scalebox{0.78}{0.427}} &\scalebox{0.78}{0.559} &\scalebox{0.78}{0.515} & \scalebox{0.78}{0.954} & \scalebox{0.78}{0.723} &\scalebox{0.78}{{0.437}} &\scalebox{0.78}{{0.449}} &\scalebox{0.78}{0.526} &\scalebox{0.78}{0.516} &\scalebox{0.78}{0.450} &\scalebox{0.78}{0.459} \\ %&\scalebox{0.78}{4.431} &\scalebox{0.78}{1.729} \\
%     \midrule
    
%     \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{ECL}}} 
%     &  \scalebox{0.78}{96} & \boldres{\scalebox{0.78}{0.148}} & \boldres{\scalebox{0.78}{0.240}} & \scalebox{0.78}{0.201} & \scalebox{0.78}{0.281} & \scalebox{0.78}{0.195} & \scalebox{0.78}{0.285} & \scalebox{0.78}{0.219} & \scalebox{0.78}{0.314} & \scalebox{0.78}{0.237} & \scalebox{0.78}{0.329} &\secondres{\scalebox{0.78}{0.168}} &\secondres{\scalebox{0.78}{0.272}} &\scalebox{0.78}{0.197} &\scalebox{0.78}{0.282} & \scalebox{0.78}{0.247} & \scalebox{0.78}{0.345} &\scalebox{0.78}{0.193} &\scalebox{0.78}{0.308} &{\scalebox{0.78}{0.169}} &{\scalebox{0.78}{0.273}} &\scalebox{0.78}{0.201} &\scalebox{0.78}{0.317}  \\ %&\scalebox{0.78}{0.274} &\scalebox{0.78}{0.368} \\
%     & \scalebox{0.78}{192} & \boldres{\scalebox{0.78}{0.162}} & \boldres{\scalebox{0.78}{0.253}} & \scalebox{0.78}{0.201} & \secondres{\scalebox{0.78}{0.283}} & \scalebox{0.78}{0.199} & \scalebox{0.78}{0.289} & \scalebox{0.78}{0.231} & \scalebox{0.78}{0.322} & \scalebox{0.78}{0.236} & \scalebox{0.78}{0.330} &{\scalebox{0.78}{0.184}} &\scalebox{0.78}{0.289} &\scalebox{0.78}{0.196} &{\scalebox{0.78}{0.285}} & \scalebox{0.78}{0.257} & \scalebox{0.78}{0.355} &\scalebox{0.78}{0.201} &\scalebox{0.78}{0.315} &\secondres{\scalebox{0.78}{0.182}} &\scalebox{0.78}{0.286} &\scalebox{0.78}{0.222} &\scalebox{0.78}{0.334} \\ %&\scalebox{0.78}{0.296} &\scalebox{0.78}{0.386} \\
%     & \scalebox{0.78}{336} & \boldres{\scalebox{0.78}{0.178}} & \boldres{\scalebox{0.78}{0.269}} & \scalebox{0.78}{0.215} & \secondres{\scalebox{0.78}{0.298}} & \scalebox{0.78}{0.215} & \scalebox{0.78}{0.305} & \scalebox{0.78}{0.246} & \scalebox{0.78}{0.337} & \scalebox{0.78}{0.249} & \scalebox{0.78}{0.344} &\secondres{\scalebox{0.78}{0.198}} &{\scalebox{0.78}{0.300}} &\scalebox{0.78}{0.209} &{\scalebox{0.78}{0.301}} & \scalebox{0.78}{0.269} & \scalebox{0.78}{0.369} &\scalebox{0.78}{0.214} &\scalebox{0.78}{0.329} &{\scalebox{0.78}{0.200}} &\scalebox{0.78}{0.304} &\scalebox{0.78}{0.231} &\scalebox{0.78}{0.338}  \\ %&\scalebox{0.78}{0.300} &\scalebox{0.78}{0.394} \\
%     & \scalebox{0.78}{720} & \secondres{\scalebox{0.78}{0.225}} & \boldres{\scalebox{0.78}{0.317}} & \scalebox{0.78}{0.257} & \scalebox{0.78}{0.331} & \scalebox{0.78}{0.256} & \scalebox{0.78}{0.337} & \scalebox{0.78}{0.280} & \scalebox{0.78}{0.363} & \scalebox{0.78}{0.284} & \scalebox{0.78}{0.373} &\boldres{\scalebox{0.78}{0.220}} &\secondres{\scalebox{0.78}{0.320}} &\scalebox{0.78}{0.245} &\scalebox{0.78}{0.333} & \scalebox{0.78}{0.299} & \scalebox{0.78}{0.390} &\scalebox{0.78}{0.246} &\scalebox{0.78}{0.355} &{\scalebox{0.78}{0.222}} &{\scalebox{0.78}{0.321}} &\scalebox{0.78}{0.254} &\scalebox{0.78}{0.361} \\ %&\scalebox{0.78}{0.373} &\scalebox{0.78}{0.439} \\
%     \cmidrule(lr){2-24}
%     & \scalebox{0.78}{Avg} & \boldres{\scalebox{0.78}{0.178}} & \boldres{\scalebox{0.78}{0.270}} & \scalebox{0.78}{0.219} & \scalebox{0.78}{0.298} & \scalebox{0.78}{0.216} & \scalebox{0.78}{0.304} & \scalebox{0.78}{0.244} & \scalebox{0.78}{0.334} & \scalebox{0.78}{0.251} & \scalebox{0.78}{0.344} &\secondres{\scalebox{0.78}{0.192}} &\secondres{\scalebox{0.78}{0.295}} &\scalebox{0.78}{0.212} &\scalebox{0.78}{0.300} & \scalebox{0.78}{0.268} & \scalebox{0.78}{0.365} &\scalebox{0.78}{0.214} &\scalebox{0.78}{0.327} &{\scalebox{0.78}{0.193}} &{\scalebox{0.78}{0.296}} &\scalebox{0.78}{0.227} &\scalebox{0.78}{0.338} \\ %&\scalebox{0.78}{0.311} &\scalebox{0.78}{0.397} \\
%     \midrule

%     % \multirow{5}{*}{\rotatebox{90}{\update{\scalebox{0.95}{Exchange}}}}
%     % &  \scalebox{0.78}{96} & \boldres{\scalebox{0.78}{0.086}} & \secondres{\scalebox{0.78}{0.206}} & \scalebox{0.78}{0.093} & \scalebox{0.78}{0.217} & \secondres{\scalebox{0.78}{0.088}} & \boldres{\scalebox{0.78}{0.205}} & \scalebox{0.78}{0.256} & \scalebox{0.78}{0.367} & \scalebox{0.78}{0.094} & \scalebox{0.78}{0.218} & \scalebox{0.78}{0.107} & \scalebox{0.78}{0.234} & \scalebox{0.78}{0.088} & \scalebox{0.78}{0.218} & \scalebox{0.78}{0.267} & \scalebox{0.78}{0.396} & \scalebox{0.78}{0.148} & \scalebox{0.78}{0.278} & \scalebox{0.78}{0.111} & \scalebox{0.78}{0.237} & \scalebox{0.78}{0.197} & \scalebox{0.78}{0.323} \\ %& \scalebox{0.78}{0.847} & \scalebox{0.78}{0.752} \\
%     % &  \scalebox{0.78}{192} & \scalebox{0.78}{0.177} & \secondres{\scalebox{0.78}{0.299}} & \scalebox{0.78}{0.184} & \scalebox{0.78}{0.307} & \boldres{\scalebox{0.78}{0.176}} & \boldres{\scalebox{0.78}{0.299}} & \scalebox{0.78}{0.470} & \scalebox{0.78}{0.509} & \scalebox{0.78}{0.184} & \scalebox{0.78}{0.307} & \scalebox{0.78}{0.226} & \scalebox{0.78}{0.344} & \secondres{\scalebox{0.78}{0.176}} & \scalebox{0.78}{0.315} & \scalebox{0.78}{0.351} & \scalebox{0.78}{0.459} & \scalebox{0.78}{0.271} & \scalebox{0.78}{0.315} & \scalebox{0.78}{0.219} & \scalebox{0.78}{0.335} & \scalebox{0.78}{0.300} & \scalebox{0.78}{0.369} \\ %& \scalebox{0.78}{1.204} & \scalebox{0.78}{0.895} \\
%     % &  \scalebox{0.78}{336} & \scalebox{0.78}{0.331} & \secondres{\scalebox{0.78}{0.417}} & \scalebox{0.78}{0.351} & \scalebox{0.78}{0.432}& \boldres{\scalebox{0.78}{0.301}} & \boldres{\scalebox{0.78}{0.397}} & \scalebox{0.78}{1.268} & \scalebox{0.78}{0.883} & \scalebox{0.78}{0.349} & \scalebox{0.78}{0.431} & \scalebox{0.78}{0.367} & \scalebox{0.78}{0.448} & \secondres{\scalebox{0.78}{0.313}} & \scalebox{0.78}{0.427} & \scalebox{0.78}{1.324} & \scalebox{0.78}{0.853} & \scalebox{0.78}{0.460} & \scalebox{0.78}{0.427} & \scalebox{0.78}{0.421} & \scalebox{0.78}{0.476} & \scalebox{0.78}{0.509} & \scalebox{0.78}{0.524} \\ %& \scalebox{0.78}{1.672} & \scalebox{0.78}{1.036} \\
%     % &  \scalebox{0.78}{720} & \secondres{\scalebox{0.78}{0.847}} & \boldres{\scalebox{0.78}{0.691}} & \scalebox{0.78}{0.886} & \scalebox{0.78}{0.714} & \scalebox{0.78}{0.901} & \scalebox{0.78}{0.714} & \scalebox{0.78}{1.767} & \scalebox{0.78}{1.068} & \scalebox{0.78}{0.852} & \scalebox{0.78}{0.698} & \scalebox{0.78}{0.964} & \scalebox{0.78}{0.746} & \boldres{\scalebox{0.78}{0.839}} & \scalebox{0.78}{0.695} & \scalebox{0.78}{1.058} & \scalebox{0.78}{0.797} & \scalebox{0.78}{1.195} & \secondres{\scalebox{0.78}{0.695}} & \scalebox{0.78}{1.092} & \scalebox{0.78}{0.769} & \scalebox{0.78}{1.447} & \scalebox{0.78}{0.941} \\ %& \scalebox{0.78}{2.478} & \scalebox{0.78}{1.310} \\
%     % \cmidrule(lr){2-24}
%     % &  \scalebox{0.78}{Avg} & \secondres{\scalebox{0.78}{0.360}} & \boldres{\scalebox{0.78}{0.403}} & \scalebox{0.78}{0.378} & \scalebox{0.78}{0.417} & \scalebox{0.78}{0.367} & \secondres{\scalebox{0.78}{0.404}} & \scalebox{0.78}{0.940} & \scalebox{0.78}{0.707} & \scalebox{0.78}{0.370} & \scalebox{0.78}{0.413} & \scalebox{0.78}{0.416} & \scalebox{0.78}{0.443} & \boldres{\scalebox{0.78}{0.354}} & \scalebox{0.78}{0.414} & \scalebox{0.78}{0.750} & \scalebox{0.78}{0.626} & \scalebox{0.78}{0.519} & \scalebox{0.78}{0.429} & \scalebox{0.78}{0.461} & \scalebox{0.78}{0.454} & \scalebox{0.78}{0.613} & \scalebox{0.78}{0.539} \\ %& \scalebox{0.78}{1.550} & \scalebox{0.78}{0.998} \\


%     %\midrule
    
%     \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{Traffic}}} 
%     & \scalebox{0.78}{96} & \boldres{\scalebox{0.78}{0.395}} & \boldres{\scalebox{0.78}{0.268}} & \scalebox{0.78}{0.649} & \scalebox{0.78}{0.389} & \scalebox{0.78}{0.544} & \scalebox{0.78}{0.359} & \secondres{\scalebox{0.78}{0.522}} & \secondres{\scalebox{0.78}{0.290}} & \scalebox{0.78}{0.805} & \scalebox{0.78}{0.493} &{\scalebox{0.78}{0.593}} &{\scalebox{0.78}{0.321}} &\scalebox{0.78}{0.650} &\scalebox{0.78}{0.396} & \scalebox{0.78}{0.788} & \scalebox{0.78}{0.499} &{\scalebox{0.78}{0.587}} &\scalebox{0.78}{0.366} &\scalebox{0.78}{0.612} &{\scalebox{0.78}{0.338}} &\scalebox{0.78}{0.613} &\scalebox{0.78}{0.388} \\ %&\scalebox{0.78}{0.719} &\scalebox{0.78}{0.391}\\
%     & \scalebox{0.78}{192} & \boldres{\scalebox{0.78}{0.417}} & \boldres{\scalebox{0.78}{0.276}} & \scalebox{0.78}{0.601} & \scalebox{0.78}{0.366} & \scalebox{0.78}{0.540} & \scalebox{0.78}{0.354} & \secondres{\scalebox{0.78}{0.530}} & \secondres{\scalebox{0.78}{0.293}} & \scalebox{0.78}{0.756} & \scalebox{0.78}{0.474} &\scalebox{0.78}{0.617} &{\scalebox{0.78}{0.336}} &{\scalebox{0.78}{0.598}} &\scalebox{0.78}{0.370} & \scalebox{0.78}{0.789} & \scalebox{0.78}{0.505} &\scalebox{0.78}{0.604} &\scalebox{0.78}{0.373} &\scalebox{0.78}{0.613} &{\scalebox{0.78}{0.340}} &\scalebox{0.78}{0.616} &\scalebox{0.78}{0.382}  \\ %&\scalebox{0.78}{0.696} &\scalebox{0.78}{0.379} \\
%     & \scalebox{0.78}{336} & \boldres{\scalebox{0.78}{0.433}} & \boldres{\scalebox{0.78}{0.283}} & \scalebox{0.78}{0.609} & \scalebox{0.78}{0.369} & \secondres{\scalebox{0.78}{0.551}} & \scalebox{0.78}{0.358} & \scalebox{0.78}{0.558} & \secondres{\scalebox{0.78}{0.305}}  & \scalebox{0.78}{0.762} & \scalebox{0.78}{0.477} &\scalebox{0.78}{0.629} &{\scalebox{0.78}{0.336}}  &{\scalebox{0.78}{0.605}} &\scalebox{0.78}{0.373} & \scalebox{0.78}{0.797} & \scalebox{0.78}{0.508}&\scalebox{0.78}{0.621} &\scalebox{0.78}{0.383} &\scalebox{0.78}{0.618} &{\scalebox{0.78}{0.328}} &\scalebox{0.78}{0.622} &\scalebox{0.78}{0.337} \\ %&\scalebox{0.78}{0.777} &\scalebox{0.78}{0.420} \\
%     & \scalebox{0.78}{720} & \boldres{\scalebox{0.78}{0.467}} & \boldres{\scalebox{0.78}{0.302}} & \scalebox{0.78}{0.647} & \scalebox{0.78}{0.387} & \secondres{\scalebox{0.78}{0.586}} & \scalebox{0.78}{0.375} & \scalebox{0.78}{0.589} & \secondres{\scalebox{0.78}{0.328}}  & \scalebox{0.78}{0.719} & \scalebox{0.78}{0.449} &\scalebox{0.78}{0.640} &{\scalebox{0.78}{0.350}} &\scalebox{0.78}{0.645} &\scalebox{0.78}{0.394} & \scalebox{0.78}{0.841} & \scalebox{0.78}{0.523} &{\scalebox{0.78}{0.626}} &\scalebox{0.78}{0.382} &\scalebox{0.78}{0.653} &{\scalebox{0.78}{0.355}} &\scalebox{0.78}{0.660} &\scalebox{0.78}{0.408} \\ %&\scalebox{0.78}{0.864} &\scalebox{0.78}{0.472} \\
%     \cmidrule(lr){2-24}
%     & \scalebox{0.78}{Avg} & \boldres{\scalebox{0.78}{0.428}} & \boldres{\scalebox{0.78}{0.282}} & \scalebox{0.78}{0.626} & \scalebox{0.78}{0.378} & \scalebox{0.78}{0.555} & \scalebox{0.78}{0.362} & \secondres{\scalebox{0.78}{0.550}} & \secondres{\scalebox{0.78}{0.304}} & \scalebox{0.78}{0.760} & \scalebox{0.78}{0.473} &{\scalebox{0.78}{0.620}} &{\scalebox{0.78}{0.336}} &\scalebox{0.78}{0.625} &\scalebox{0.78}{0.383} & \scalebox{0.78}{0.804} & \scalebox{0.78}{0.509} &{\scalebox{0.78}{0.610}} &\scalebox{0.78}{0.376} &\scalebox{0.78}{0.624} &{\scalebox{0.78}{0.340}} &\scalebox{0.78}{0.628} &\scalebox{0.78}{0.379} \\ %&\scalebox{0.78}{0.764} &\scalebox{0.78}{0.416} \\
%     \midrule
    
%     \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{Weather}}} 
%     &  \scalebox{0.78}{96} & \scalebox{0.78}{0.174} & \boldres{\scalebox{0.78}{0.214}} & \scalebox{0.78}{0.192} & \scalebox{0.78}{0.232} & \scalebox{0.78}{0.177} & \secondres{\scalebox{0.78}{0.218}} & \boldres{\scalebox{0.78}{0.158}} & \scalebox{0.78}{0.230}  & \scalebox{0.78}{0.202} & \scalebox{0.78}{0.261} &\secondres{\scalebox{0.78}{0.172}} &{\scalebox{0.78}{0.220}} & \scalebox{0.78}{0.196} &\scalebox{0.78}{0.255} & \scalebox{0.78}{0.221} & \scalebox{0.78}{0.306} & \scalebox{0.78}{0.217} &\scalebox{0.78}{0.296} & {\scalebox{0.78}{0.173}} &{\scalebox{0.78}{0.223}} & \scalebox{0.78}{0.266} &\scalebox{0.78}{0.336} \\ %& \scalebox{0.78}{0.300} &\scalebox{0.78}{0.384}  \\
%     & \scalebox{0.78}{192} & \scalebox{0.78}{0.221} & \boldres{\scalebox{0.78}{0.254}} & \scalebox{0.78}{0.240} & \scalebox{0.78}{0.271} & \scalebox{0.78}{0.225} & \scalebox{0.78}{0.259} & \boldres{\scalebox{0.78}{0.206}} & \scalebox{0.78}{0.277} & \scalebox{0.78}{0.242} & \scalebox{0.78}{0.298} &\secondres{\scalebox{0.78}{0.219}} &\secondres{\scalebox{0.78}{0.261}}  & \scalebox{0.78}{0.237} &\scalebox{0.78}{0.296} & \scalebox{0.78}{0.261} & \scalebox{0.78}{0.340} & \scalebox{0.78}{0.276} &\scalebox{0.78}{0.336} & \scalebox{0.78}{0.245} &\scalebox{0.78}{0.285} & \scalebox{0.78}{0.307} &\scalebox{0.78}{0.367} \\ %& \scalebox{0.78}{0.598} &\scalebox{0.78}{0.544} \\
%     & \scalebox{0.78}{336} & \secondres{\scalebox{0.78}{0.278}} & \boldres{\scalebox{0.78}{0.296}} & \scalebox{0.78}{0.292} & \scalebox{0.78}{0.307} & \scalebox{0.78}{0.278} & \secondres{\scalebox{0.78}{0.297}} & \boldres{\scalebox{0.78}{0.272}} & \scalebox{0.78}{0.335} & \scalebox{0.78}{0.287} & \scalebox{0.78}{0.335} &{\scalebox{0.78}{0.280}} &{\scalebox{0.78}{0.306}} & \scalebox{0.78}{0.283} &\scalebox{0.78}{0.335} & \scalebox{0.78}{0.309} & \scalebox{0.78}{0.378} & \scalebox{0.78}{0.339} &\scalebox{0.78}{0.380} & \scalebox{0.78}{0.321} &\scalebox{0.78}{0.338} & \scalebox{0.78}{0.359} &\scalebox{0.78}{0.395}\\ % &\scalebox{0.78}{0.578} &\scalebox{0.78}{0.523} \\
%     & \scalebox{0.78}{720} & \scalebox{0.78}{0.358} & \boldres{\scalebox{0.78}{0.349}} & \scalebox{0.78}{0.364} & \scalebox{0.78}{0.353} & \secondres{\scalebox{0.78}{0.354}} & \secondres{\scalebox{0.78}{0.348}} & \scalebox{0.78}{0.398} & \scalebox{0.78}{0.418} & \boldres{\scalebox{0.78}{0.351}} & \scalebox{0.78}{0.386} &\scalebox{0.78}{0.365} &{\scalebox{0.78}{0.359}} & {\scalebox{0.78}{0.345}} &{\scalebox{0.78}{0.381}} & \scalebox{0.78}{0.377} & \scalebox{0.78}{0.427} & \scalebox{0.78}{0.403} &\scalebox{0.78}{0.428} & \scalebox{0.78}{0.414} &\scalebox{0.78}{0.410} & \scalebox{0.78}{0.419} &\scalebox{0.78}{0.428} \\ %& \scalebox{0.78}{1.059} &\scalebox{0.78}{0.741} \\
%     \cmidrule(lr){2-24}
%     & \scalebox{0.78}{Avg} & \boldres{\scalebox{0.78}{0.258}} & \boldres{\scalebox{0.78}{0.279}} & \scalebox{0.78}{0.272} & \scalebox{0.78}{0.291} & \secondres{\scalebox{0.78}{0.259}} & \secondres{\scalebox{0.78}{0.281}} & \scalebox{0.78}{0.259} & \scalebox{0.78}{0.315} & \scalebox{0.78}{0.271} & \scalebox{0.78}{0.320} &{\scalebox{0.78}{0.259}} &{\scalebox{0.78}{0.287}} &\scalebox{0.78}{0.265} &\scalebox{0.78}{0.317} & \scalebox{0.78}{0.292} & \scalebox{0.78}{0.363} &\scalebox{0.78}{0.309} &\scalebox{0.78}{0.360} &\scalebox{0.78}{0.288} &\scalebox{0.78}{0.314} &\scalebox{0.78}{0.338} &\scalebox{0.78}{0.382} \\ %&\scalebox{0.78}{0.634} &\scalebox{0.78}{0.548} \\
%     \midrule
    
%     % \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{Solar-Energy}}} 
%     % &  \scalebox{0.78}{96} &\boldres{\scalebox{0.78}{0.203}} &\boldres{\scalebox{0.78}{0.237}} & \scalebox{0.78}{0.322} & \scalebox{0.78}{0.339} & \secondres{\scalebox{0.78}{0.234}} & \secondres{\scalebox{0.78}{0.286}} &\scalebox{0.78}{0.310} &\scalebox{0.78}{0.331} &\scalebox{0.78}{0.312} &\scalebox{0.78}{0.399} &\scalebox{0.78}{0.250} &\scalebox{0.78}{0.292} &\scalebox{0.78}{0.290} &\scalebox{0.78}{0.378} &\scalebox{0.78}{0.237} &\scalebox{0.78}{0.344} &\scalebox{0.78}{0.242} &\scalebox{0.78}{0.342} &\scalebox{0.78}{0.215} &\scalebox{0.78}{0.249} &\scalebox{0.78}{0.884} &\scalebox{0.78}{0.711}\\ % &\scalebox{0.78}{0.236} &\secondres{\scalebox{0.78}{0.259}} \\
%     % & \scalebox{0.78}{192} &\boldres{\scalebox{0.78}{0.233}} &\boldres{\scalebox{0.78}{0.261}} & \scalebox{0.78}{0.359} & \scalebox{0.78}{0.356}& \secondres{\scalebox{0.78}{0.267}} & \secondres{\scalebox{0.78}{0.310}} &\scalebox{0.78}{0.734} &\scalebox{0.78}{0.725} &\scalebox{0.78}{0.339} &\scalebox{0.78}{0.416} &\scalebox{0.78}{0.296} &\scalebox{0.78}{0.318} &\scalebox{0.78}{0.320} &\scalebox{0.78}{0.398} &\scalebox{0.78}{0.280} &\scalebox{0.78}{0.380} &\scalebox{0.78}{0.285} &\scalebox{0.78}{0.380} &\scalebox{0.78}{0.254} &\scalebox{0.78}{0.272} &\scalebox{0.78}{0.834} &\scalebox{0.78}{0.692} \\ %&\boldres{\scalebox{0.78}{0.217}} &\secondres{\scalebox{0.78}{0.269}} \\
%     % & \scalebox{0.78}{336} &\boldres{\scalebox{0.78}{0.248}} &\boldres{\scalebox{0.78}{0.273}} & \scalebox{0.78}{0.397} & \scalebox{0.78}{0.369}& \secondres{\scalebox{0.78}{0.290}}  &\secondres{\scalebox{0.78}{0.315}} &\scalebox{0.78}{0.750} &\scalebox{0.78}{0.735} &\scalebox{0.78}{0.368} &\scalebox{0.78}{0.430} &\scalebox{0.78}{0.319} &\scalebox{0.78}{0.330} &\scalebox{0.78}{0.353} &\scalebox{0.78}{0.415} &\scalebox{0.78}{0.304} &\scalebox{0.78}{0.389} &\scalebox{0.78}{0.282} &\scalebox{0.78}{0.376} &\scalebox{0.78}{0.290} &\scalebox{0.78}{0.296} &\scalebox{0.78}{0.941} &\scalebox{0.78}{0.723} \\ %&\secondres{\scalebox{0.78}{0.249}} &\secondres{\scalebox{0.78}{0.283}}\\
%     % & \scalebox{0.78}{720} &\boldres{\scalebox{0.78}{0.249}} &\boldres{\scalebox{0.78}{0.275}} & \scalebox{0.78}{0.397} & \scalebox{0.78}{0.356} & \secondres{\scalebox{0.78}{0.289}} &\secondres{\scalebox{0.78}{0.317}} &\scalebox{0.78}{0.769} &\scalebox{0.78}{0.765} &\scalebox{0.78}{0.370} &\scalebox{0.78}{0.425} &\scalebox{0.78}{0.338} &\scalebox{0.78}{0.337} &\scalebox{0.78}{0.356} &\scalebox{0.78}{0.413} &\scalebox{0.78}{0.308} &\scalebox{0.78}{0.388} &\scalebox{0.78}{0.357} &\scalebox{0.78}{0.427} &\scalebox{0.78}{0.285} &\scalebox{0.78}{0.295} &\scalebox{0.78}{0.882} &\scalebox{0.78}{0.717} \\ %&\boldres{\scalebox{0.78}{0.241}} &\boldres{\scalebox{0.78}{0.317}}\\
%     % \cmidrule(lr){2-24}
%     % & \scalebox{0.78}{Avg} &\boldres{\scalebox{0.78}{0.233}} &\boldres{\scalebox{0.78}{0.262}} & \scalebox{0.78}{0.369} & \scalebox{0.78}{0.356} &\secondres{\scalebox{0.78}{0.270}} &\secondres{\scalebox{0.78}{0.307}} &\scalebox{0.78}{0.641} &\scalebox{0.78}{0.639} &\scalebox{0.78}{0.347} &\scalebox{0.78}{0.417} &\scalebox{0.78}{0.301} &\scalebox{0.78}{0.319} &\scalebox{0.78}{0.330} &\scalebox{0.78}{0.401} &\scalebox{0.78}{0.282} &\scalebox{0.78}{0.375} &\scalebox{0.78}{0.291} &\scalebox{0.78}{0.381} &\scalebox{0.78}{0.261} &\scalebox{0.78}{0.381} &\scalebox{0.78}{0.885} &\scalebox{0.78}{0.711} \\ %&\secondres{\scalebox{0.78}{0.235}} &\secondres{\scalebox{0.78}{0.280}}\\
%     % \midrule
%       \multicolumn{2}{c|}{\scalebox{0.78}{{$1^{\text{st}}$ Count}}} & \scalebox{0.78}{\boldres{16}} & \scalebox{0.78}{\boldres{22}} & \scalebox{0.78}{6} & \scalebox{0.78}{\secondres{12}} & \scalebox{0.78}{\secondres{12}} & \scalebox{0.78}{11} & \scalebox{0.78}{3} & \scalebox{0.78}{0} & \scalebox{0.78}{1} & \scalebox{0.78}{0} & \scalebox{0.78}{1} & \scalebox{0.78}{0} & \scalebox{0.78}{2} & \scalebox{0.78}{0} & \scalebox{0.78}{0} & \scalebox{0.78}{0} & \scalebox{0.78}{4} & \scalebox{0.78}{0} & \scalebox{0.78}{0} & \scalebox{0.78}{0} & \scalebox{0.78}{0} & \scalebox{0.78}{0} \\ %& \scalebox{0.78}{2} & \scalebox{0.78}{1}\\
%     \bottomrule
%   \end{tabular}
%     \end{small}
%   \end{threeparttable}
% %}
% \end{table*}



==> section/intro.tex <==
\section{Introduction}
Multivariate time series forecasting plays a pivotal role in diverse applications such as weather prediction~\cite{angryk2020multivariate}, energy consumption~\cite{demirel2012forecasting}, healthcare~\cite{matsubara2014funnel}, and traffic flow estimation~\cite{li2017diffusion}. 
In the field of multivariate time series forecasting, two typical approaches have emerged: historical-value-based~\cite{zhou2021informer,wu2021autoformer, zeng2023transformers, nie2022time}, and time-index-based models~\cite{woo2023learning,naour2023time}. 
Historical-value-based models predict future time steps utilizing historical observations, $\hat{x}_{t+1}=f_{\theta}(x_{t}, x_{t-1},...)$, while time-index-based models only  use the corresponding time-index features, $\hat{x}_{t+1}=f_{\theta}(t+1)$. 
Historical-value-based models have been widely explored due to their simplicity and effectiveness, making them the state-of-the-art models in the field. 
However, it is important to acknowledge that multivariate time series data are often discretely sampled from continuous dynamical systems. This characteristic poses a challenge for historical-value-based models, as they tend to capture spurious correlations limited to the sampling frequency~\cite{gong2017causal, woo2023learning}.
Moreover, despite their widespread use and effectiveness, the progress in developing historical-value-based models has encountered bottlenecks~\cite{li2023revisiting}, making it challenging to further improve their performance. This limitation motivates the exploration of alternative approaches that can overcome the shortcomings of historical-value-based models and potentially deliver more robust forecasting models.

In recent years, deep time-index-based models have gradually been studied~\cite{woo2023learning,naour2023time}. These models intrinsically avoid the aforementioned problem of historical-value-based models, by mapping the time-index features to target predictions in continuous space through implicit neural representations~\cite{tancik2020fourier,sitzmann2020implicit} (INRs). 
However, time-index-based models are only characterized by time-index coordinates, which makes them ineffective in modeling complex time series data and lacking in exploratory capabilities.

% In recent years, the research on deep time-index-based models has gained attention~\cite{woo2023learning,naour2023time}. These models offer an intrinsic solution to the limitations of historical-value-based models by mapping time-index features to target predictions in continuous space through implicit neural representations (INRs)~\cite{tancik2020fourier,sitzmann2020implicit}
% However, by solely relying on time-index coordinates, these models may struggle to effectively model complex time series data and lack the exploratory capabilities of historical-value-based models. This is because they do not explicitly consider the spatial dependencies and interactions between variables in the time series.
%Different from previous works that aggregate the feature of spatial domains (historical-value-based models) or temporal domains (time-index-based models), we treat multivariate time series as spatiotemporal data discretely sampled from a continuous dynamical system, 
%Different from previous works, we treat multivariate time series as spatiotemporal data discretely sampled from a continuous dynamical system, 
In this work, we propose a novel perspective by treating multivariate time series as spatiotemporal data discretely sampled from a continuous dynamical system, described by partial differential equations (PDEs) with fixed spatial domains as described in Eq~\ref{eq:pde_def}. 

From the PDE perspective, we observe that historical-value-based and time-index-based models can be considered as simplified versions of Eq~\ref{eq:pde}, where either the temporal or spatial information is removed.

By examining Eq~\ref{eq:pde}, we can interpret historical-value-based models as implicit inverse problems. These models infer spatial domain information, such as the position and physical properties of sensors, from historical observations. By utilizing the initial condition and spatial domain information, these models predict future sequences. Mathematically, historical-value-based models can be formulated as:
\begin{align}
    \hat{x}_{\tau}=x_{\tau_{0}}+ \int_{\tau_{0}}^{\tau} f_{\theta}(x) d\tau
\end{align}
where $x$ represents the spatial domain information.

Time-index-based models, on the other hand, can be seen as models that consider only the temporal domain. These models solely rely on time-index coordinates for prediction and do not explicitly incorporate spatial information. In this case, the prediction is formulated as:
\begin{align}
    \hat{x}_{\tau}= \int_{\tau_{0}}^{\tau} f_{\theta}(t_{\tau}) d\tau
\end{align}

% From the PDE perspective, the training objectives of historical-value-based and time-index-based models are implicitly defined as (For historical-value-based models, they can be viewed as implicit inverse problems, where the models infer spatial domain information (e.g., the position and physical properties of sensors) from historical observations. Using the initial condition and spatial domain information, these models predict future sequences, which can be formulated as $\hat{x}_{\tau}=\int_{\tau_{0}}^{\tau} f_{\theta}(x_{his}) d \tau\approx x_{\tau_{0}}+\int_{\tau_{0}}^{\tau}f_{\theta}(x) d \tau$, where $x$ represents the spatial domain information. ):
% %which can be represented by a complex partial differential equation (PDE) with the spatial domain being fixed. 
% %which is commonly described with partial differential equations (PDEs) with the spatial domains being fixed as described in Equation~\ref{eq:pde_def}. From the perspective of PDEs, the training objective of historical-value-based and time-index-based models are implicitly defined as :
% \begin{align}
%     %\mathcal{L}_{h}&=\mathcal{L}(x_{\tau},\int_{\tau_{0}}^{\tau} f_{\theta}(x_{his}) d \tau) \\
%     \mathcal{L}_{h}&=\mathcal{L}(x_{\tau},x_{\tau_{0}}+\int_{\tau_{0}}^{\tau} f_{\theta}(x) d \tau) \\
%     \mathcal{L}_{t}&=\mathcal{L}(x_{\tau},\int_{\tau_{0}}^{\tau}f_{\theta}(t_{\tau})d \tau)
% \end{align}
% where $\tau$ is the time-index, $x_{his}$ is the spatial feature, and $t_{\tau}$ is the temporal feature. 
% We observe that historical-value-based and time-index-based models can be considered as simplified versions of  Eq~\ref{eq:pde}, where either the temporal or spatial information is removed.

%We found that historical-value-based and time-index-based models are simplified terms of Eq~\ref{eq:pde} that remove temporal or spatial information.

Motivated by the limitations of existing approaches and inspired by neural PDE solvers, we introduce PDETime, a PDE-based model for LMTF. PDETime considers LMTF as an Initial Value Problem, explicitly incorporating both spatial and temporal domains and requiring the specification of an initial condition. 
%PDETime encompasses both historical-value-based and time-index-based models as special cases, where either the spatial or temporal domain is considered, respectively.

% For the historical-value-based models, we consider them as implicit inverse problems where they implicitly infer spatial domain information (e.g. the position and physical properties of sensors) from historical observations and use the initial condition and spatial domains information to predict future sequence which can be formulated as $\hat{x}_{\tau}=x_{\tau_{0}}+\int_{\tau_{0}}^{\tau}f_{\theta}(x) d \tau$, where $x$ refers spatial domains information. 
% For historical-value-based models, they can be viewed as implicit inverse problems, where the models infer spatial domain information (e.g., the position and physical properties of sensors) from historical observations. Using the initial condition and spatial domain information, these models predict future sequences, which can be formulated as $\hat{x}_{\tau}=x_{\tau_{0}}+\int_{\tau_{0}}^{\tau}f_{\theta}(x) d \tau$, where $x$ represents the spatial domain information.

% In this work, we consider LMTF as Initial Value problems, which can be described by Equation~\ref{eq:pde}, where $x_{\tau_{0}}$ at any time $t_{\tau_{0}}$ is required to infer $x_{\tau}$ for $\tau > \tau_{0}$.
% Therefore, PDE-based methods consider both the spatial and temporal domains and need to explicitly specify the initial condition. 
% Obviously, PDE-based models encompass both historical-value-based and time-index-based models as special cases, where either the spatial domain or the temporal domain is considered, respectively.
%Obviously, historical-value-based and time-index-based models are special cases of PDE-based models, using spatial domains or temporal domains, respectively.

%Based on the motivations discussed above, and drawing inspiration from neural PDE solvers, we propose PDETime, a PDE-based model for LMTF, as depicted in Figure~\ref{fig:pdetime}.
Specifically, PDETime first predicts the partial derivative term $E_{\theta}(x_{his},t_{\tau})=\alpha_{\tau} \approx\frac{\partial u(x,t_{\tau})}{\partial t_{\tau}}$ utilizing an encoder in latent space. Unlike traditional PDE problems, the spatial domain information of LMT is unknown. Therefore, the encoder utilizes historical observations to estimate the spatial domain information. Subsequently, a numerical solver is employed to calculate the integral term $z_{\tau}=\int_{\tau_{0}}^{\tau} \alpha_{\tau} d\tau$. The proposed solver effectively mitigates the error issue and enhances the stability of the prediction results compared to traditional ODE solvers~\cite{chen2018neural}. Finally, PDETime employs a decoder to map the integral term from the latent space to the spatial domains and predict the results as $\hat{x}_{\tau}=x_{\tau_{0}}+D_{\phi}(z_{\tau})$. Similar to time-index-based models, PDETime also utilizes meta-optimization to enhance its ability to extrapolate across the forecast horizon. Additionally, PDETime can be simplified into a historical-value-based or time-index-based model by discarding either the time or spatial domains, respectively. 


% inspired by neural PDE solvers, we propose PDETime, a PDE-based model, for 
% %long-term multivariate time-series forecasting
% LMTF. Given the initial condition $x_{\tau_{0}}$ and target time $t_{\tau}$, PDETime predicts the target series by performing the following encoding, integration, and decoding operations. More specifically, PDETime first predict the partial term $E_{\theta}(x_{his},t_{\tau})=\alpha_{\tau} \approx\frac{\partial u(x,t_{\tau})}{\partial t_{\tau}}$ utilizing a encoder in latent space. Different from traditional PDE problems, the spatial domain information of LMT is unknown. Thus, the encoder uses historical observations to fit the spatial domain information. After, a numerical solver is used to calculate the integral term $z_{\tau}=\int_{\tau_{0}}^{\tau} \alpha_{\tau} d\tau$. Compared with traditional ODE Solvers~\cite{chen2018neural}, the proposed solver can effectively alleviate the error problem and make the prediction results more stable. Finally, PDETime uses a decoder to map integral term from the latent space to spatial domains and predict the results $\hat{x}_{\tau}=x_{\tau_{0}}+D_{\phi}(z_{\tau})$.
% %$\alpha_{\tau} =\frac{\partial u(x,t_{\tau})}{\partial t_{\tau}}$ ,$z_{\tau}=\int_{\tau_{0}}^{\tau} \alpha_{\tau} d\tau$, $x_{\tau}=x_{\tau_{0}}+D_{\phi}(z_{\tau})$ 
% Like time-index-based models, PDETime also utilizes meta-optimization to enhance the ability to extrapolate across the forecast horizon. PDETime can also degenerate into historical-value-based or time-index-based model by discarding the temporal domains or the spatial domains.

In short, we summarize the key contributions of this work:
%The contributions are summarized as follows:

\begin{itemize}
    %\item We rethink the long-term multivariate time-series forecasting as Initial Value Problem of PDEs and introduce a novel PDE-based model for LMTF.
    % \item We rethink the long-term multivariate time series as the spatiotemporal data regularly sampled from PDEs along the temporal domains.
    % \item We treat the LMTF as the Initial Value Problem of PDEs and introduce PDETime, a novel PDE-based model inspired by neural PDE solvers. PDETime follows the encoding-integration-decoding operations and utilizes the meta-optimization to extrapolate future series.
    % %\item We Develop PDETime, a , inspired by neural PDE solvers
    % \item We conduct extensive experiments under the long-term setting over seven real-world benchmarks across multiple domains. Our empirical studies show that the proposed model has achieved consistent state-of-the-art performance.
    \item We propose a novel perspective for LMTF by considering it as spatiotemporal data regularly sampled from PDEs along the temporal domains.
    \item We introduce PDETime, a PDE-based model inspired by neural PDE solvers, which tackles LMTF as an Initial Value Problem of PDEs. PDETime incorporates encoding-integration-decoding operations and leverages meta-optimization to extrapolate future series.
    \item We extensively evaluate the proposed model on seven real-world benchmarks across multiple domains under the long-term setting. Our empirical studies demonstrate that PDETime consistently achieves state-of-the-art performance.
\end{itemize}

==> section/related_work.tex <==
\section{Related Work}
\textbf{Multivariate Time Series Forecasting.} 
With the progressive breakthrough made in deep learning, deep models have been proposed to tackle various time series forecasting applications. Depending on whether temporal or spatial is utilized, these models are classified into historical-value-based~\cite{zhou2021informer, zhou2022fedformer, zeng2023transformers, nie2022time, zhang2022crossformer,liu2023itransformer, liu2022non, liu2022scinet, wu2022timesnet}, and time-index-based models~\cite{woo2023learning}. Historical-value-based models, predicting target time steps utilizing historical observations, have been extensively developed and made significant progress in which a large body of work that tries to apply Transformer to forecast long-term series in recent years~\cite{wen2023transformers}. 
% Early works~\cite{zhou2021informer, wu2021autoformer} were focused on designing novel mechanism to reduce the complexity of the original attention mechanism, thus capturing long-term dependency to achieve better performance. 
Early works like Informer~\cite{zhou2021informer} and LongTrans~\cite{li2019enhancing} were focused on designing novel mechanism to reduce the complexity of the original attention mechanism, thus capturing long-term dependency to achieve better performance. Afterwards, efforts were made to extract better temporal features to enhance the performance of the model~\cite{wu2021autoformer,zhou2022fedformer}. %Autoformer~\cite{wu2021autoformer} uses auto-correlation to get patch level connectionts. FEDformer~\cite{zhou2022fedformer} employs the mixture-of-expert design to enhance the seasonal-trend decomposition and presents a sparse attention within the frequency domains. 
Recent work~\cite{zeng2023transformers} has found that a single linear channel-independent model can outperform complex transformer-based models. Therefore, the very recent channel-independent models like PatchTST~\cite{nie2022time} and DLinear~\cite{zeng2023transformers} have become state-of-the-art. 
In contrast, time-index-based models~\cite{woo2023learning, fons2022hypertime,jiang2023nert,naour2023time} are a kind of coordinated-based models, mapping coordinates to values, which was represented by INRs. These models have received less attention and their performance still lags behind historical-value-based models.
%In contrast to historical-value-based models, time-index-based models have been recently introduced and explored to a lesser extent. 
PDETime, unlike previous works, considers multivariate time series as spatiotemporal data and approaches the prediction target sequences from the perspective of partial differential equations (PDEs).

%In contrast, time-index-based models have not been thoroughly investigated, and their performance still lags behind that of historical-value-based models. 


\textbf{Implicit Neural Representations.} Implicit Neural Representations are the class of works representing signals as a continuous function parameterized by multi-layer perceptions (MLPs)~\cite{tancik2020fourier, sitzmann2020implicit} (instead of using the traditional discrete representation). These neural networks have been used to learn differentiable representations of various objects such as images~\cite{henzler2020learning}, shapes~\cite{liu2020dist,liu2019learning}, and textures~\cite{oechsle2019texture}. However, there is limited research on INRs for times series~\cite{fons2022hypertime,jiang2023nert,woo2023learning, naour2023time,jeong2022time}. And previous works mainly focused on time series generation and anomaly detection~\cite{fons2022hypertime, jeong2022time}. 
DeepTime~\cite{woo2023learning} is the work designed to learn a set of basis INR functions for forecasting, however, its performance is worse than historical-value-based models. In this work, we use INRs to represent spatial domains and temporal domains.

%\textbf{Deep Learning for PDEs.} Physics-informed neural networks (PINNs)~\cite{} have demonstrated that PDEs can be accurately solved via neural networks.

\textbf{Neural PDE Solvers.} Neural PDE solvers which are used for temporal PDEs, are laying the foundations of what is becoming both a rapidly growing and impactful area of research. These neural PDE solvers fall into two broad categories, \textit{neural operator methods} and \textit{autoregressive methods}. The neural operator methods~\cite{kovachki2021neural,li2020fourier,lu2021learning} treat the mapping from initial conditions to solutions as time $t$ as an input-output mapping learnable via supervised learning. For a given PDE and given initial conditions $u_{0}$, the neural operator $\mathcal{M}$ is trained to satisfy $\mathcal{M}(t, u_{0})=u(t)$. However, these methods are not designed to generalize to dynamics for out-of-distribution $t$. In contrast, the autoregressive methods~\cite{bar2019learning, greenfeld2019learning, hsieh2019learning, yin2022continuous, brandstetter2021message} solve the PDEs iteratively. The solution of autoregressive methods at time $t+ \Delta t$ as $u(t+ \Delta)=\mathcal{A}(u(t), \Delta t)$. In this work, We consider multivariate time series as data sampled from a continuous dynamical system according to a regular time discretization, which can be described by partial differential equations. For the given initial condition $x_{\tau_{0}}$, we use the numerous solvers (Euler solver) to simulate target time step $x_{\tau}$.
%Implicit Neural Representations (INRs~\cite{}) are the class of coordinate-based neural networks which use the fully connected networks as continuous, memory-efficient implicit representations for images~\cite{}, or 3D scenes~\cite{}.

%Implicit Neural Representations (INRs~\cite{} ) are the class of works representing signals as a continuous function parameterized by neural networks (instead of using the traditional discrete representation)

